Vertical Federated Learning without Revealing Intersection Membership

Vertical Federated Learning (vFL) allows multiple parties that own different attributes (e.g. features and labels) of the same data entity (e.g. a person) to jointly train a model. To prepare the training data, vFL needs to identify the common data entities shared by all parties. It is usually achieved by Private Set Intersection (PSI) which identifies the intersection of training samples from all parties by using personal identifiable information (e.g. email) as sample IDs to align data instances. As a result, PSI would make sample IDs of the intersection visible to all parties, and therefore each party can know that the data entities shown in the intersection also appear in the other parties, i.e. intersection membership. However, in many real-world privacy-sensitive organizations, e.g. banks and hospitals, revealing membership of their data entities is prohibited. In this paper, we propose a vFL framework based on Private Set Union (PSU) that allows each party to keep sensitive membership information to itself. Instead of identifying the intersection of all training samples, our PSU protocol generates the union of samples as training instances. In addition, we propose strategies to generate synthetic features and labels to handle samples that belong to the union but not the intersection. Through extensive experiments on two real-world datasets, we show our framework can protect the privacy of the intersection membership while maintaining the model utility.

==> Backup/tex/additional_experiments.tex <==
\section{Additional Experiments}
\subsection{Criteo}

\begin{figure*}[t]
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo/cut_layer_norm_attack_mean_test_auc_trade_off.pdf}
      \caption*{ (a: )}
  \end{minipage}
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo/cut_layer_hint_attack_hints_5_norm_mean_test_auc_trade_off.pdf}
    \caption*{(b: )}
  \end{minipage}
   \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo/cut_layer_hint_attack_hints_5_inner_product_mean_test_auc_trade_off.pdf}
      \caption*{ (c: )}
  \end{minipage}
 \vspace{-1.5em}
 \caption{Criteo: trade-off between test AUC and leak AUC. num hints = $5$.}
 \label{fig:criteo_tradeoff_test_auc_privacy} 
\end{figure*}

\begin{figure*}[t]
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo/cut_layer_norm_attack_mean_test_loss_trade_off.pdf}
      \caption*{ (a: )}
  \end{minipage}
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo/cut_layer_hint_attack_hints_5_norm_mean_test_loss_trade_off.pdf}
    \caption*{(b: )}
  \end{minipage}
   \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo/cut_layer_hint_attack_hints_5_inner_product_mean_test_loss_trade_off.pdf}
      \caption*{ (c: )}
  \end{minipage}
 \vspace{-1.5em}
 \caption{Criteo: trade-off between test loss and leak AUC. num hints = $5$.}
 \label{fig:criteo_tradeoff_test_loss_privacy} 
\end{figure*}


\begin{figure*}[ht!]
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/num_hints/criteo/sumKL_mean_ip_leak_test_auc.pdf}
      \caption*{ (a: )}
  \end{minipage}
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/num_hints/criteo/sumKL_mean_norm_leak_test_auc.pdf}
    \caption*{(b: )}
  \end{minipage}
  \medskip
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/num_hints/criteo/white_gaussian_mean_ip_leak_test_auc.pdf}
      \caption*{ (c: )}
  \end{minipage}
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/num_hints/criteo/white_gaussian_mean_norm_leak_test_auc.pdf}
    \caption*{(d: )}
  \end{minipage}
 \caption{Criteo: effects of num hints on the cut layer}
 \label{fig:criteo_num_hints} 
\end{figure*}


\begin{figure*}[ht!]
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/layer_position/criteo/norm_attack_sumKL_layer_position.pdf}
      \caption*{ (a: norm\_attack\_sumKL\_layer\_position)}
  \end{minipage}
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/layer_position/criteo/norm_attack_white_gaussian_layer_position.pdf}
    \caption*{(b: norm\_attack\_white\_gaussian\_layer\_position)}
  \end{minipage}
  \medskip
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/layer_position/criteo/sumKL_mean_hint_norm_attack_layer_position.pdf}
      \caption*{ (c:sumKL\_mean\_hint\_norm\_attack\_layer\_position )}
  \end{minipage}
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/layer_position/criteo/white_gaussian_mean_hint_norm_attack_layer_position.pdf}
    \caption*{(d: white\_gaussian\_mean\_hint\_norm\_attack\_layer\_position)}
  \end{minipage}
  \medskip
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/layer_position/criteo/sumKL_mean_hint_ip_attack_layer_position.pdf}
      \caption*{ (e:sumKL\_mean\_hint\_ip\_attack\_layer\_position )}
  \end{minipage}
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/layer_position/criteo/white_gaussian_mean_hint_ip_attack_layer_position.pdf}
    \caption*{(f: white\_gaussian\_mean\_hint\_ip\_attack\_layer\_position)}
  \end{minipage}
 \caption{Criteo: effects of layer position}
 \label{fig:criteo_layer_position} 
\end{figure*}

\begin{figure*}[ht!]
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/against_different_attack_methods/sumKL_against_different_attack_methods.pdf}
      \caption*{ (a: sumKL_against_different_attack_methods)}
  \end{minipage}
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/against_different_attack_methods/white_gaussian_against_different_attack_methods.pdf}
    \caption*{(b: white_gaussian_against_different_attack_methods)}
  \end{minipage}
 \caption{Criteo: against different attack methods}
 \label{fig:criteo_aginst_different_attack_methods} 
\end{figure*}



\begin{figure*}[t]
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/avazu/cut_layer_norm_attack_mean_test_auc_trade_off.pdf}
      \caption*{ (a: )}
  \end{minipage}
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/avazu/cut_layer_hint_attack_hints_5_norm_mean_test_auc_trade_off.pdf}
    \caption*{(b: )}
  \end{minipage}
   \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/avazu/cut_layer_hint_attack_hints_5_inner_product_mean_test_auc_trade_off.pdf}
      \caption*{ (c: )}
  \end{minipage}
 \vspace{-1.5em}
 \caption{Avazu: trade-off between test AUC and leak AUC. num hints = $5$.}
 \label{fig:avazu_tradeoff_test_auc_privacy} 
\end{figure*}



\begin{figure*}[t]
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/avazu/cut_layer_norm_attack_mean_test_loss_trade_off.pdf}
      \caption*{ (a: )}
  \end{minipage}
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/avazu/cut_layer_hint_attack_hints_5_norm_mean_test_loss_trade_off.pdf}
    \caption*{(b: )}
  \end{minipage}
   \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/avazu/cut_layer_hint_attack_hints_5_inner_product_mean_test_loss_trade_off.pdf}
      \caption*{ (c: )}
  \end{minipage}
 \vspace{-1.5em}
 \caption{Avazu: trade-off between test loss and leak AUC. num hints = $5$.}
 \label{fig:avazu_tradeoff_test_loss_privacy} 
\end{figure*}





==> Backup/tex/conclusion.tex <==
\section{Conclusion}
In this paper, we identify a simple norm-based method to uncover the private labels of the active party using the communicated gradients in the two-party split learning problem for binary classification. We then propose a theoretically principled method to determine the best additive random perturbation to the gradients to reduce the probability of label leakage against a general class of label uncovering methods. We also conducted extensive experiments to demonstrate the effectiveness of our proposed protection methods. 

% We note that label leakage in the gradient-sharing scheme is a general phenomenon, as long as the gradient distributions are not identical for different labels, and prior knowledge on these distributions is known to the passive party.
We note that label leakage in the gradient-sharing scheme is a general phenomenon, as long as prior knowledge on the gradient distributions is known to the passive party.
It remains open if the passive party can computational efficiently exploit this leakage when cryptographic scheme is applied in the learning protocol like in \cite{ahtw16,kswxj18}.
Another open problem is whether there exist other methods to uncover the label information from the gradients of not necessarily imbalanced datasets and understanding how our method could protect against those attacks theoretically and empirically.  
Finally, our protection technique \marvell \,is designed to maximize the overall detection error. %over the gradient distribution. 
It would be interesting to see if similar ideas can be used to satisfy other protection requirements.
%what type of protection we could achieve for the label leakage on individual instances.


% \begin{comment}
\textbf{Acknowledgements} We would like to express our thanks to the team members at ByteDance for providing the collaborative federated learning framework, Fedlearner\footnote{\url{https://github.com/bytedance/fedlearner}}. In addition, we would like to thank Liangchao Wu, Di Wu, and Xiaobing Liu for their discussions and supports. The code is availale at {\url {https://github.com/bytedance/fedlearner/tree/master/example/privacy/label_protection}}.
% \end{comment}

==> Backup/tex/experiments.tex <==
\label{sec:experiment}

\subsection{Experimental Settings}

% \subsection{Public benchmark datasets}

In this section, we evaluate the proposed gradient perturbation methods on the
%FMINIST \footnote{\url{https://deepobs.readthedocs.io/en/stable/api/datasets/fmnist.html}} \footnote{We change it to binary classification problem by randomly selecting some instances in a class as positive ones, and considering all the left instances as negative ones.} and
Criteo%~\cite{criteo}
\footnote{{https://www.kaggle.com/c/criteo-display-ad-challenge/data}} 
and Avazu%~\cite{avazu}
\footnote{{https://www.kaggle.com/c/avazu-ctr-prediction/data}} 
 dataset. Criteo is a real-world large-scale binary classification dataset with approximately $45$ million user click records in online advertising. Avazu contains approximately $40$ million entries ($11$ days of clicks/not clicks of Avazu data).
Both datasets are highly imbalanced: $25\%$ of the Criteo and $17\%$ of the Avazu data is in the positive class.
We split each dataset randomly into two parts: with $90\%$ for training and the rest for tests. We train a Wide\&Deep model \cite{cheng2016wide} where the passive party consists of embedding layers for input features and four layers of $128$-unit ReLU activated multilayer perceptron (deep part) and the active party consists of the last two layers of the deep part and the entire wide part of the model. In every iteration, the passive party sends a mini-batch of $1, 024$ examples' $128$-dimensional vector to the active party and the active party sends the gradients of the loss w.r.t. these vectors back to the passive side. %We train the model for 30 epochs.

% \subsection{Comparison partners}
We compare our proposed protection techniques (\maxnorm{} \ and \marvell) with a baseline named  {\tt iso}, \ where i.i.d. isotropic Gaussian noise is added to every gradient example $g$ in the communicated mini-batch. Every $g_i$ in the batch of size $B$ is added with {$\calN(0, {(s/d)\cdot \max_{i=1}^B \norm{g_i}_2^2}I_{d \times d})$}, where $s$ is a parameter to tune. 

% \subsection{Evaluation metric}
We quantitatively measure the model's utility and privacy by the AUC of the ROC. The value is estimated at every gradient update iteration using the mini-batch examples. Higher leak AUC means the label is leaked more likely to leak by the communicated gradients. A model with good trade-off between utility and privacy should have a high-performance AUC (low test loss) and a leak AUC close to $0.5$ (random guess). 

%\vspace{-0.125in}
\subsection{Robustness of Marvell}

\begin{figure*}[ht!]
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/layer4_leak_auc.pdf}
    \caption*{\scriptsize(a)}
  \end{minipage}
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/layer1_leak_auc.pdf}
      \caption*{\scriptsize (b)}
  \end{minipage}
  \begin{minipage}[b]{0.33\linewidth}
    \centering
    {\small
    % \begin{tabular}{r|c|c|c}
    %      & no noise & iso & sumKL \\ 
    %   \hline\hline train loss & 0.4067 & 0.4700 & 0.4672 \\
    %     test AUC & 0.8062 & 0.7921 & 0.7949\\
    %     \hline & \multicolumn{3}{c}{max leak AUC}\\
    %     layer1 & 1.0000 & 0.5536 & 0.5554 \\
    %     layer2 & 1.0000 & 0.5652 & 0.5583 \\
    %     layer3 & 1.0000 & 0.6089 & 0.5710 \\
    %     layer4 & 1.0000 & 0.5129 & 0.5188\\
    %     \multicolumn{4}{c}{} \\
    %     \multicolumn{4}{c}{}
    % \end{tabular}
%     \begin{table}[!htp]\centering
    \begin{tabular}{l|c|cr}\toprule
    &Parameters & ACE \\\midrule
    \multirow{4}{*}{Marvell} &0.1 &0.01170 \\
    &0.2 &0.01167 \\
    &0.3 &0.01159 \\
    &0.4 &0.01187 \\ \midrule
    \maxnorm{} &- &0.01184 \\ \midrule
    iso &1.0 &0.01178 \\ \midrule
    no\_noise &- &0.01148 \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-2.0em}
    \caption*{\scriptsize (c)}
    %\captionsetup[figure]{labelformat=empty}
  \end{minipage} 
%   \begin{minipage}[b]{0.5\linewidth}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/tradeoff.pdf}
%     % \vspace{-2.0em}
%     \caption*{(d)}
%   \end{minipage}
  \vspace{-1.5em}
 \caption{Figure (a) and (b) shows the leak AUC of no protection training and  Marvell with different values of lower bound $L = [0.1, 0.2, 0.3, 0.4]$ at the cut layer (layer 4) and a previous layer (layer 1) respectively on Criteo. Figure (c): Comparing  Marvell and  \maxnorm{}  with the baseline method iso on ACE. In all the figures/table, no\_noise is the standard training with no gradient perturbation as protection.}
 \label{fig:experiments} 
%  \vspace{-0.2in}
\end{figure*}

In this section, we show the robustness of \marvell \ on protecting different layers of the model and its effects on the corresponding model's reliability. 

In Figure \ref{fig:experiments}(a), we plot the leak AUC for every batch of communicated gradient at the cut layer (layer 4) throughout the entire training. We see that with no gradient perturbation, the leak AUC is consistently around $0.9$ through the majority of training. On the other hand, when using our proposed technique (\marvell), we see a large reduction in leak AUC. The leak AUC becomes lower (more privacy protection) when we impose a higher lower bound $L$ for the worst-case detection error. In addition, it is natural to ask whether the gradients of the layers before the cut layer can also leak the label information as the passive party keeps back propagating towards the first layer. In Figure \ref{fig:experiments} (b), we plot the leak AUC of the first layer's activation gradients for the same set of methods shown in Figure \ref{fig:experiments} (a)---the leak AUC is at the same high level for the no protection method, indicating that previous layer's gradients could also leak the label information. However, our method with different lower bound $L$ can still significantly reduce the leak AUC even though the protection was analyzed at the cut layer.

Adaptive Calibration Error (ACE) ~\cite{ACE2019} can measure how well a model’s predicted probabilities of outcomes reflect true probabilities of those outcomes. We report the ACE in Figure \ref{fig:experiments} (c) to show that different perturbation methods have little effect on the reliability of the corresponding model’s confidence in its predictions. \marvell \ and \maxnorm{} can have similar ACE as \nonoise, demonstrating that our proposed protection methods' robustness on the model's reliability of prediction. 

%\vspace{-0.125in}
\subsection{Trade-off between Utility and Privacy}

\begin{figure*}[ht!]
\vspace{-0.1in}
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo/cut_layer_norm_attack_mean_test_auc_trade_off.pdf}
      \caption*{ (a: norm attack on Criteo)}
  \end{minipage}
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo/cut_layer_hint_attack_hints_5_inner_product_mean_test_loss_trade_off.pdf}
    \caption*{(b: hint attack on Criteo)}
  \end{minipage}
   \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo/cut_layer_hint_attack_hints_5_inner_product_mean_test_auc_trade_off.pdf}
      \caption*{ (c: hint attack on Criteo)}
  \end{minipage}
  \medskip
    \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/avazu/cut_layer_norm_attack_mean_test_auc_trade_off.pdf}
      \caption*{(d: norm attack on Avazu )}
  \end{minipage}
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/avazu/cut_layer_hint_attack_hints_5_inner_product_mean_test_loss_trade_off.pdf}
    \caption*{(e: hint attack on Avazu)}
  \end{minipage}
   \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/avazu/cut_layer_hint_attack_hints_5_inner_product_mean_test_auc_trade_off.pdf}
      \caption*{ (f: hint attack on Avazu)}
  \end{minipage}
\vspace{-0.1in}
 \caption{
 Figure (a) shows the trade-off between leak AUC (norm attack) and test AUC on Criteo. Figure (b) and (c) shows the trade-off between leak AUC (hint attack) and test loss and test AUC on Criteo respectively. Figure (d), (e), and (f) show the corresponding trade-offs on Avazu dataset. Each point represents a utility and privacy performance with a specific setting (for example $s$ for \iso \ and sumKL for \marvell). Since \maxnorm{} \ and \nonoise \ has no parameter to tune, they have only one point in the corresponding Figures. We set the number of hints as $5$ and use inner product to compute the pairwise distance for hint attack. 
 }
 \label{fig:utility_privacy_tradeoff} 
\vspace{-0.15in}
\end{figure*}

\begin{figure*}[ht!]
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/live_experiments/norm_attack_leak_roc_auc.pdf}
      \caption*{(a: Leak AUC of Norm Attack)}
  \end{minipage}
  \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/live_experiments/hint_attack_leak_roc_auc.pdf}
    \caption*{(b: Leak AUC of Hint Attack)}
  \end{minipage}
   \begin{minipage}[b]{0.33\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/live_experiments/roc_auc.pdf}
      \caption*{ (c: Performance AUC)}
  \end{minipage}
 \vspace{-1.5em}
 \caption{Figure (a) and (b) shows different protection methods' leak AUC of norm attack and hint attack respectively at the cut layer. Figure (c) shows different protection methods' performance AUC. The x-asix represents the date (ranging from Jan. to Feb. 2020), and the y-axis represents the corresponding daily average utility and privacy.}
 \label{fig:live_experiments} 
  \vspace{-0.25in}
\end{figure*}


\begin{comment}
\begin{figure}[ht!]
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo_epoch_5_norm_attack_tradeoff.pdf}
      \caption*{ (a: Norm Attack on Criteo)}
  \end{minipage}
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo_epoch_5_hint_attack_tradeoff.pdf}
    \caption*{(b: Hint Attack on Criteo)}
  \end{minipage}
  \medskip
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/live_experiments/avazu_norm_attack_tradeoff.pdf}
      \caption*{ (c: Norm Attack on Avazu)}
  \end{minipage}
  \begin{minipage}[b]{0.495\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/live_experiments/avazu_hint_attack_tradeoff.pdf}
    \caption*{(d: Hint Attack on Avazu)}
  \end{minipage}
 \caption{Figure (a) and (c) shows the trade-off between utility and privacy (norm attack) on Criteo and Avazu dataset respectively. Figure (b) and (d) shows the trade-off between utility and privacy (hint attack) on Criteo and Avazu dataset respectively. Each point represents a utility and privacy performance with a specific setting (for example $s$ for \iso \ and sumKL for \marvell). Since \maxnorm{} \ and \nonoise \ has no parameter to tune, they have only one point in the corresponding Figures.}
 \label{fig:utility_privacy_tradeoff} 
%  \vspace{-0.25in}
\end{figure}
\end{comment}
%%%%%%%%%%%Figures of Live Experiments are Put here to get the expected position. 

In this section, we show that \marvell \ and \maxnorm{} \ can achieve a trade-off between model performance (utility) and privacy more easily than \iso \ under the \normattack. In addition, we would also like to test our proposed protection methods' effectiveness on preventing label leakage against some extreme scenarios. We introduce an attack method named as {\tt hint attack} that is powerful but difficult to deploy in reality. \hintattack \ assumes that the passive party knows some positive instances (working as hints)\footnote{The passive party cannot use the hints repeatedly in different mini-batches, since it can be detected by the active party easily.} in each communicated mini-batch during training, and the passive party can compute the pairwise distance (inner product/cosine similarity for example) %\footnote{Other distance metrics such as Euclidean distance can achieve the similar effects as inner product in our experiments. Due to the space limit, we only report using inner product in our paper.} 
between hints and unknown label instances based on their corresponding gradients. An instance will be assigned a positive label if it is close to any hint. In our experiments, \hintattack \ with the number of hints set as $5$ makes the leak AUC be close to $1.0$ on both Criteo and Avazu datasets. It's worth mentioning that hint attack with inner product is still effective for balanced datasets, since positive and negative gradients have opposite directions even in balanced datasets. 

As shown in Figure~\ref{fig:utility_privacy_tradeoff}, the x-axis represents the corresponding model's leak AUC (the closer to be $0.5$ the better) under some attack, and the y-axis reflects the corresponding model's performance (evaluated by test AUC on Figure (c) and (f) and test loss on Figure (b) and (e)) at the same time. %Each point represents a utility and privacy performance with a specific setting (for example $s$ for \iso \ and sumKL for \marvell). Since \maxnorm{} and \nonoise \ has no parameter to tune, they have only one point in the corresponding Figures. 
Generally speaking, a protection technique that can achieve good trade-off between test AUC and privacy should fall into the upper-left area of the figure. We observe that in Figure ~\ref{fig:utility_privacy_tradeoff} (a) and (d) that \marvell \ and \maxnorm{} achieves better trade-off between test AUC and leak AUC than \iso \ on preventing the norm attack. %Particularly, \maxnorm{} can achieve the best trade-off among all the protection methods regarding to the norm attack, since \maxnorm{} is designed to prevent norm attack. 
However, \maxnorm{} becomes less effective than \marvell \ when dealing with the hint attack, as shown in Figure~\ref{fig:utility_privacy_tradeoff} (b), (c), (e), and (f). A model that can achieve a good trade-off between test loss and privacy should fall into the lower-left area of the figure. %Figure (b) and (e) shows the trade-off between leak AUC and test loss of different protection techniques defending hint attack on Criteo and Avazu dataset respectively. 
In this case, \marvell{} achieves the best trade-off between leak AUC and test loss on both Criteo and Avazu as shown in Figure ~\ref{fig:utility_privacy_tradeoff} (b) and (e) respectively. Also, since we do not optimize AUC directly, it is possible to observe that \iso{} has a worse test loss than \marvell{} but has a similar (but not better) test AUC as \marvell{}.
%Overall, Figure~\ref{fig:utility_privacy_tradeoff} demonstrates that \marvell \ as a theoretically principled method to determine the best additive random perturbation to the gradients can reduce the probability of label leakage under both norm and hint attacks and achieve reasonable utility at the same time.
Overall, as shown in Figure~\ref{fig:utility_privacy_tradeoff}, \marvell{} has achieved smaller test loss and higher test AUC with approximately the same if not better leak AUC than \maxnorm{} and \iso{}. 
This demonstrates that the optimization-based model achieves a better utility privacy trade-off than other comparison partners. 


% Lastly, we analyze how our technique compares to a baseline method where i.i.d. isotropic Gaussian noise is added to every gradient example $g$ in the communicated mini-batch. Because we care about a strong level of label protection, we compare our method that has the strongest privacy requirement $L=0.4$ against a white Gaussian baseline where every $g_i$ in the batch of size $B$ is added with {\scriptsize$\calN(0, \frac{25\cdot \max_{i=1}^B \norm{g_i}_2^2}{d}I_{d \times d})$}.


% We show the end-of-training loss, the best test AUC, and each deep layer's leak AUC value in Figure 2(c). As we can see, our proposed perturbation has achieved smaller training loss and higher test AUC while also having approximately the same if not better leak AUC. This shows that our optimization-based model has achieved a better privacy performance trade-off than adding isotropic Gaussian noise.

\begin{comment}
\begin{figure*}[h!] %
  \begin{minipage}[b]{0.245\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo_epoch_5_norm_attack_tradeoff.pdf}
    \vspace{-2.0em}
    \caption*{(a: Norm Attack on Criteo)}
  \end{minipage}
%   \vspace{2em}
  \begin{minipage}[b]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/tradeoff/criteo_epoch_5_hint_attack_tradeoff.pdf}
    \vspace{-2.0em}
    \caption*{(b: Hint Attack on Criteo)}
    %\captionsetup[figure]{labelformat=empty}
  \end{minipage} 
  \begin{minipage}[b]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/live_experiments/avazu_norm_attack_tradeoff.pdf}
    \vspace{-2.0em}
    \caption*{(c: Norm Attack on Avazu)}
  \end{minipage} 
  \begin{minipage}[b]{0.245\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/live_experiments/avazu_hint_attack_tradeoff.pdf}
    \vspace{-2.0em}
    \caption*{(d: Hint Attack on Criteo)}
  \end{minipage} 
  \vspace{-0.5em}
 \caption{...}
 \label{fig:utility_privacy_tradeoff}
\end{figure*}

\begin{figure*}
    \includegraphics[width=0.95\textwidth]{figures/experiment_results.pdf}
    \caption{.}
    \label{fig:experiment_results}
\end{figure*}
\begin{figure*}
    \includegraphics[width=0.5\textwidth]{figures/test_auclayer1_leak_auc.pdf}
    \caption{.}
    \label{fig:experiment_results}
\end{figure*}
\begin{figure*}
    \includegraphics[width=0.5\textwidth]{figures/train_losslayer1_leak_auc.pdf}
    \caption{.}
    \label{fig:experiment_results}
\end{figure*}
\end{comment}



==> Backup/tex/framework.tex <==
\label{sec:framework}
In this section we first formally describe the gradient-based two-party split learning problem for imbalanced binary classification.
%With this setup, we give a simple framework to think about raw data leakage in split learning.
A careful inspection of the distribution of the communicated gradients in this setting allows us to identify an effective method to uncover the active party's labels.

%\WH{I think the problem setting/problem abstraction of split learning is not our novel contribution. We can use fewer words to introduce the problem setting and use more words on Section 2.1.}

% \vspace{-0.125in}
\subsection{Split Learning on Binary Classification}

Consider two parties learning a model for a binary classification problem over the domain $\calX \times \cbrck{0, 1}$. Here the passive and active parties want to learn a composition model $h \circ f$ jointly, where the raw features $X$ and $f: \calX \to \Real^d$ are stored on the passive party side while the labels $y$ and $h: \Real^d \to \Real$ is on the active party side. Let $\ell = h(f(X))$ be the logit of the positive class where the positive class's predicted probability is given by the sigmoid function as follows: $\widetilde{p}_1 = 1/(1 + \exp(-\ell))$. The loss of the model is given by the cross entropy $L = \log(1 + \exp(-\ell)) + (1 - y)\ell$. During the model inference, the passive party computes $f(X)$ and sends it to the active party who will then compute the rest of computation (Forward in Table \ref{tab:model_training}). \footnote{
%In this formulation, we don't allow the active party to add any additional features to compute the logit. This is an assumption that simplifies the notation and derivation but as we shall see still keep the data leakage problem real and interesting enough. 
For the simplifying of the notation and derivation, we add no additional features in the active party to compute the logit. The data leakage problem still holds true for other complicated settings (see in the experiment section).
} 

To train the model using gradient descent, the active party starts the gradient computation process by first computing the gradient of the loss w.r.t. the logit $\frac{dL}{d\ell} = (\widetilde{p}_1 - y)$. Using the chain rule, the active party can then compute the gradient of $L$ with respect to $h$'s parameters through $\ell$. In order to allow the passive party to learn $f$, the active party also computes the gradient of $L$ with respect to the input of the function $h$. We denote this gradient by $g \coloneqq \nabla_{f(X)} L = (\widetilde{p}_1 - y) \nabla_a h(a) \vert_{a = f(X)} \in \Real^d$  (equality by chain rule). After receiving $g$ sent from the active party, the passive party can compute the gradient of $L$ w.r.t. $f$'s parameters (Backward in Table \ref{tab:model_training}). Since the gradient $g$ sent to the passive party is a function of both $f(X)$ and $y$, it is possible that $g$ could contain information about the label $y$.

%(we temporarily denote this dependence through $g = g(f(X), y)$ At any point during the training, with $f$ and $g$ fixed, the communicated feature $f(X)$ and $g(f(X), y)$ can be thought of as functions of the random variables $(X, y)$ drawn from the data distribution. As a result, the data distribution \textbf{induces a distribution of the four random variables} $(X, \;  f(X),\; g(f(X),y),\; y)$. The passive party has access to samples of the first three variables (but not the label $y$) for every training example while the active party has access to the last three variables (but not the input $X$). Because there is likely correlation these random variables, it is conceptually possible to use the values of three to infer that of the other -- based on the correlation, the passive party infer $y$ while the active party could infer $X$. In this paper, we will only consider protecting the active party's label $y$ from the passive party by reducing the correlation of $g$ with $y$.

% \newcommand{\pp}{c}
  \begin{table*}[!ht]
  \centering
%   \begin{center}
    % \scriptsize
    \begin{tabular}{ cccccccccc }
      { Forward:} & $X$ & $\xrightarrow{\bm{f}}$ & $\bm{f}(X)$ & $\stackrel{\textrm{\scriptsize comm.}}{\Longrightarrow}$ & $\bm{f}(X)$ & $\xrightarrow{\bm{h}}$ &$\ell=h(f(X))$ & $\rightarrow$ & $\stackrel{\stackrel{\mbox{$y$}}{\downarrow}}{L}$ \\
      { Backward:} & & & $g$ & $\stackrel{\textrm{\scriptsize comm.}}{\Longleftarrow}$ & $g $ & $\leftarrow$ & $\frac{dL}{dl} = (\widetilde{p}_1 - y)$ & $\leftarrow$ & $1$ \\
      & & & $\downarrow$ & & & & $\downarrow$ & & \\
      & & & $f$'s param & & & & $h$'s param & & 
    \end{tabular}
%   \end{center}
    \caption{Communication diagram of model training ($\leftarrow$ and $\downarrow$ represent gradient computation using the chain rule).}
    \label{tab:model_training}
    \vspace{-0.15in}
  \end{table*}

When $B$ examples are forwarded as a batch, the communicated features $f(X)$ and gradients $g$ will both be matrices of shape $\Real^{B \times d}$ with each row belonging to a specific example in the batch. It is important to note that here the gradients as rows of the matrix are gradients of the loss with respect to different examples' intermediate computation results but not the model parameters; therefore, no averaging over or shuffling of the rows of the matrix can be done prior to communication for the sake of correct gradient computation of $f$'s parameters on the passive party side.

 %It is important to notice that for batched training with batch size $B$, the split layer $f(X)$ sent to the active party and the gradients $g$ sent back to the passive party will both be matrices of shape $\Real^{B \times d}$ with each row referring to a specific sample in the batch.
 
 % The gradient with respect to the parameters will be averaged across samples, but the communicated information can \textit{not} be averaged, due to the non-linearity of the models. Hence, the communicated information are \textit{non-aggregated}, which is different from most other federated learning scenarios.
  
  %It is \textbf{important} to note that here the gradients as rows of the matrix are gradients of the loss with respect to different examples' intermediate computation results but not the model parameters; therefore, no averaging over or shuffling of the rows of the matrix can be done for the sake of correct gradient computation for $f$'s parameters on the passive party side.

==> Backup/tex/gradient_attack.tex <==
\section{Some random thoughts}
As we discussed before, although the ``gradient sharing'' scheme does not communicate labels directly, the passive party may still be able to gain non-trivial knowledge on the labels from the active party.
Take binary classification for example.
Let $P_0$ be the distribution of the gradients of the negative examples,
and $P_1$ be the distribution of the gradients of the positive examples.
As long as $P_0\neq P_1$,
with prior knowledge on $P_0$ and $P_1$,
on receiving the gradient $g$ of some example $x$,
the passive party is able to make better prediction on the label of $x$ with maximal likelihood estimation.
For a single example $x$,
we can view the advantage over random guess as the \emph{gradient-based label-leakage} of $x$.
In this work, we focus on the label leakage for the entire training data, which is the expected label leakage under the training data distribution.

Of course, the advantage against random guess depends on the distance between $P_0$ and $P_1$ and the prior information of the passive party on these distributions,
and it can be computationally expensive for the passive party to exploit the leakage. 
In practice, the gradient-based label leakage only becomes a concern when the passive party can efficiently make use of it, which is precisely the issue we will address.

We note here that gradient-based label leakage occurs as long as the passive party gets access to the real gradients, regardless of the cryptographic scheme used in the learning protocol. Actually, if the passive party has prior knowledge on the distribution of the encrypted gradients, similar label leakage also occurs. It might be more challenging to design protection with the presence of cryptosystem, though.


==> Backup/tex/gradient_perturbation.tex <==
\label{sec:protection}
In this section, we first introduce a heuristic approach designed to prevent norm attack. Then we 
talk about our theoretically justified protection technique which strategically perturbs the gradient randomly before communication. The proposed technique can protect against a large class of label-uncovering methods including but not limited to our proposed norm-based attack method.

%\vspace{-0.125in}
\subsection{A Heuristic Approach to Prevent Norm Attack}

Section \ref{sec:norm-attack} gives an existence proof that only communicating gradients but not the raw data can still leak the private label information. 
In order to protect against label leakage, the active party should communicate the essential information of the gradient without communicating the actual gradient. Random perturbation is a class of powerful such methods. Among them a simple way is to add an isotropic Gaussian noise on the gradient to mix up the distributions of gradients $g$ of positive samples and negative samples before sending them to the passive party. Larger noise will make leak AUC smaller but potentially could have a negative impact on the learned model's predictive performance.

Although adding isotropic Gaussian noise is an effective protection method, it may not be optimal due to the following two reasons. First, the gradients are vectors instead of scalars, so the direction of the noise matters. Isotropic noise might neglect this direction information. Second, due to the asymmetry of the distribution, the active party could add different noise to the positive and negative gradients. 

\input{tex/max_norm_alignment}

Beyond the norm attack, there exists a general class of uncovering methods based on the difference of gradients distributions between positive and negative samples. Motivated by the above issues of {\tt max\_norm}, we next study how to conceivably achieve a better trade-off between model performance (utility) and label protection (privacy) even under gradient distribution based attacks. Particularly, we find where the optimal trade-off exists by mathematically defining the optimization problem for the trade-off and solving the corresponding optimization problem under Gaussianity assumption of the gradients. The added Gaussian noise is optimized to achieve the best trade-off between utility and privacy even under unknown attacks. Hence, we name this protection method as {\tt Marvell} (opti\textbf{M}ized perturb\textbf{A}tion to p\textbf{R}e\textbf{VE}nt \textbf{L}abel \textbf{L}eakage).
%Motivated by the above issues of {\tt max\_norm}, we then study where the optimal trade-off exists by mathematically defining the optimization problem for the trade-off and solving the optimization problem under Gaussianity assumption of the gradients. By adding noise in a smarter way, one could conceivably achieve a better trade-off between label protection and model performance even under unknown attacks. We name this method as {\tt Marvell} (opti\textbf{M}ized perturb\textbf{A}tion to p\textbf{R}e\textbf{VE}nt \textbf{L}abel \textbf{L}eakage).

% \WH{\begin{itemize} 
%     \item  In order to protect against label leakage, we consider adding noise. isotropic Gaussian noise is the most simple approach. 
%     \item Due to the asymmetry, isotropic Gaussian may not be the optimal. We want to ask what is the ``optimal'' way of adding noise. 
%     \item We define sumKL, which is a lower bound on error probability, as the metric of protection quality. (don't need to introduce Gaussian assumption on gradients now)
%     \item Assume Gaussianity on gradients, we are able to write the optimal noise as a solution of the optimization problem. It's optimal solution is given by $\Sigma_0^*$ and $\Sigma_1^*$.
%     \item Consequence: optimal $\Sigma_0^*$ and $\Sigma_1^*$ gives lower bound of error probability as a function of sumKL. We can control hyperparameter $P$ to achieve the error we need.
%     \end{itemize}
% }
% We consider randomly perturbing the gradient $g$ to $\widetilde{g}$ before sending them to the passive party. Here we have two natural considerations for the sake of better training loss optimization convergence. \textbf{Consideration 1}: the perturbation should be unbiased $\E[\widetilde{g}\; |\; g] = g$. This ensures that the computed  gradient of $L$ with respect to $f$'s parameters is still unbiased by chain rule and linearity of expectation. \textbf{Consideration 2}: the variance of $\widetilde{g}$ conditioned on $g$, $\V[\widetilde{g}\; |\; g = v]$, should be as small as possible for any $v$. This would control the amount of variance in the stochastic gradients of the $f$'s parameters. SGD optimization theory \cite{bottou2018optimization} shows that having unbiased and low variance stochastic gradients makes the optimization converge faster and to a lower loss value, a desirable property for model training. Specifically, we consider adding Gaussian noise to the gradient $g$ prior to communication that satisfies these two considerations. For simplicity of derivation, we assume that $g$ of the positive examples follows a Gaussian distribution $\mathcal{N}(g^{(1)}, \Sigma_{+})$, while  $g$ of the negative examples follows  $\mathcal{N}(g^{(0)}, \Sigma_{-})$\footnote{Here the Gaussian distribution is on the gradients with respect to the representation ($f(X)$) but not the parameters. Thus even for neural networks whose parameter gradient is typically sparse and non-Gaussian like, it is not unreasonable to assume the representation gradient follows a Gaussian distribution. Experimentally we also see that this assumption yields good protection performance.}. We add i.i.d. zero-mean Gaussian noise with the covariance matrices $\Sigma_1$ and $\Sigma_0$ to the positive and negative examples' $g$ respectively. The \textbf{zero-mean} additive random perturbation naturally satisfies Consideration 1. By i.i.d. of the added noise, the perturbed positive gradient follows the distribution {\scriptsize $\widetilde{\Prob}^{(1)} \coloneqq \mathcal{N}(g^{(1)}, \Sigma_{+} + \Sigma_{1})$} is , while the perturbed negative gradient follows {\scriptsize $\widetilde{\Prob}^{(0)} \coloneqq \mathcal{N}(g^{(0)}, \Sigma_{-} + \Sigma_{0})$}.
% For Consideration 2, we want to choose the $\Sigma_0$ and $\Sigma_1$ with small possible trace while achieving some protection property which we will describe next.

% In this section, we show how we add Gaussian noise to $g$ to obtain $\widetilde{g}$ before sending it to the passive party, as illustrated in Table ~\ref{tab:model_training_w_protection}. We also provide an approximate theoretical guarantee for our perturbation strategy. 

% \begin{table}[h!]
%     \centering
% % \begin{center}
%     \scriptsize
%     \begin{tabular}{ \pp \pp \pp \pp \pp \pp \pp \pp \pp \pp \pp \pp}
%       {\scriptsize forward:} & $X$ & $\xrightarrow{\bm{f}}$ & $\bm{f}(X)$ & $\stackrel{\textrm{\scriptsize comm.}}{\Longrightarrow}$ & & & $\bm{f}(X)$ & $\xrightarrow{h}$ &$\ell$ & $\rightarrow$ & $L$ \\
%       {\scriptsize back.:} & & & $\blue{\widetilde{g}}$ & $\stackrel{\textrm{\scriptsize comm.}}{\Longleftarrow}$ & $\blue{\widetilde{g}}$ & \red{$\leftarrow$}  & $g$ & $\leftarrow$ & $\frac{dL}{dl} = (\tilde{p_1} - y)$ & $\leftarrow$ & $1$ \\
%       & & & $\downarrow$ & & & & & & $\downarrow$ & & \\
%       & & & $f$'s param & & & & & & $h$'s param & & 
%     \end{tabular}
% %   \end{center}
%     \caption{Forward and back propagation of model training with gradient perturbation to protect privacy}
%     \label{tab:model_training_w_protection}
% \end{table}

% \WH{Can briefly introduce some straight-forward protection methods --- add same white Gaussian noise, expectation alignment, perpendicular noise here. We can then ask a question --- what is the best trade off between noise level and label security level, and how to properly define noise level and label security level (relation with DP can be discussed here). Then we naturally go to our definition of optimization problem.}

%\vspace{-0.125in}
\subsection{Optimized Perturbation Method}

 Consider a general class of label recovering functions $\{ \I_A, A \subset \mathbb{R}^d \}$. Let $A^c:=\mathbb{R}^{d}\backslash A$ be the complement of $A$. For any set $A \subset \mathbb{R}^d$, the labelling function $\I_A: \mathbb{R}^d \to \cbrck{0, 1}$ maps the gradient $g \in A$ to the positive class 1 and $g \in A^c$ to the negative class 0. This general class of functions encompasses the aforementioned $2$-norm detection method by $A = \{g \in \mathbb{R}^d: ||g||_2 \ge t\}$ for some fixed threshold $t$. %Denote by $\widetilde{P}^{(1)}$ and $\widetilde{P}^{(0)}$ the distribution of the additively perturbed gradients $\tilde{g}^{(1)} = g^{(1)} + \noisevec^{(1)}$ and $\tilde{g}^{(0)} = g^{(0)} + \noisevec^{(0)}$ for positive samples and negative samples respectively. 
 We denote the distribution of the additively perturbed positive and negative gradients $\tilde{g}^{(1)} = g^{(1)} + \noisevec^{(1)}$ and $\tilde{g}^{(0)} = g^{(0)} + \noisevec^{(0)}$ by $\widetilde{P}^{(1)}$ and $\widetilde{P}^{(0)}$ respectively. Here $\noisevec^{(i)}$ is a zero-mean random noise vector added independently to the random gradient $g^{(i)}$ sampled from examples of class $y = i$. Having zero-mean $\noisevec^{(i)}$ ensures the perturbed gradients with respect to $f$'s parameters is unbiased. We define the \textit{detection error} of a labelling function $\I_A$ under the perturbed gradient distribution $\widetilde{P}_1$ and $\widetilde{P}_0$ to be
$ \frac{1}{2} (\widetilde{P}^{(1)}(A^c) + \widetilde{P}^{(0)}(A))$, i.e. the average of the False Negative Rate and the False Positive Rate. To protect against the worst case labelling function, the active party wants to make the worst case labelling function's detection error to be as high as possible, i.e., to solve $$
    \max_{\widetilde{P}^{(1)}, \widetilde{P}^{(0)}} \min_A \frac{1}{2} (\widetilde{P}^{(1)}(A^c) + \widetilde{P}^{(0)}(A)).$$
% \begin{align*}
%     \textrm{False Negative Rate (FNR)} = &\Prob_{\widetilde{g} \sim \tilde{P}^{(1)}}(\mathbb{I}_A(\widetilde{g}) = 0) \\
%     =& \Prob_{\widetilde{g} \sim \tilde{P}^{(1)}}(\widetilde{g} \in A^c) \\
%     =& \Prob_{\tilde{P}^{(1)}} (A^c)\\
%     \textrm{False Positive Rate (FPR)} = &\Prob_{\widetilde{g} \sim \tilde{P}^{(0)}}(\mathbb{I}_A(\widetilde{g}) = 1) \\
%     =& \Prob_{\widetilde{g} \sim \tilde{P}^{(0)}}(\widetilde{g} \in A) \\
%     =& \Prob_{\tilde{P}^{(0)}} (A).
%  \end{align*}
% Adversary (passive party) wants both FNR and FPR to be as low as possible. The mixture error probability $M(\tilde{P}^{(1)}, \tilde{P}^{(0)}, A) = 0.5 \cdot \textrm{FNR} + 0.5 \cdot \textrm{FPR}$ can be considered to evaluate the overall protection quality. The most malicious adversary chooses the region $A$ with respect to the perturbed distributions $\tilde{P}^{(1)}, \tilde{P}^{(0)}$ so that its error rate is the lowest (recover the most number of labels correctly).  Thus we define the worst case error probability as
% %   \begin{align*}
%     $\textrm{Error}(\tilde{P}^{(1)}, \tilde{P}^{(0)}) = \min_{A \subset \mathbb{R}^d} M(\tilde{P}^{(1)}, \tilde{P}^{(0)}, A).$
% %   \end{align*}
% Through some derivation, the worst case adversary error probability can be equivalently expressed as $\textrm{Error}(\tilde{P}^{(1)}, \tilde{P}^{(0)}) = \; 0.5 - 0.5 \cdot {TV}(\tilde{P}^{(1)}, \tilde{P}^{(0)})$
We can rewrite the optimization problem as $$\max_{\widetilde{P}^{(1)}, \widetilde{P}^{(0)}} \frac{1}{2}(1 - \TV(\widetilde{P}^{(1)}, \widetilde{P}^{(0)})),$$
where $\TV(\cdot, \cdot)$ is the total variation distance.
%where $\TV(\cdot, \cdot)$ is the total variation distance and the equality follows directly from $\TV$'s definition. 
Thus this is equivalent to minimizing the total variation distance between $\tilde{P}^{(1)}$ and $\tilde{P}^{(0)}$. Because the TV distance between high dimensional distributions are not tractable, we seek to minimize a tractable upper bound of the total variation distance. By applying Pinsker's inequality and Jensen's inequality, we obtain an upper bound of total variation distance by the sum of KL divergence (sumKL):
%\footnote{We use summation of KL divergences to maintain symmetry of the objective.}
 \begin{align*}
    \TV(P, Q) \le &\frac{1}{2} ( \sqrt{{\KL{P}{Q}}/{2}} + \sqrt{{\KL{Q}{P}}/{2}})\\
\le &\frac{1}{2} \sqrt{\KL{P}{Q} + \KL{Q}{P}}. 
\end{align*}Thus, our optimization objective can be written as follows.
\begin{align}
    \textrm{sumKL}^*:=\min_{\widetilde{P}^{(1)}, \widetilde{P}^{(0)}} \KL{\widetilde{P}^{(1)}}{\widetilde{P}^{(0)}} + \KL{\widetilde{P}^{(0)}}{\widetilde{P}^{(1)}}.
    \label{eq:protection_objective_sumKL}
\end{align}
% \begin{align*}
%     \min_{\Sigma_1, \Sigma_0} KL({\mathcal{N}(g^{(1)}, \Sigma_{+} + \Sigma_{1})} || {\mathcal{N}(g^{(0)}, \Sigma_{-} + \Sigma_{0})}) + KL({\mathcal{N}(g^{(0)}, \Sigma_{-} + \Sigma_{0})}{\mathcal{N}(g^{(1)} || \Sigma_{+} + \Sigma_{1})})
% \end{align*}
% \WH{Typo in the formula}
% \begin{align*}
%     TV(P, Q) \le \frac{\sqrt{\frac{KL({P}||{Q})}{2}}+ \sqrt{\frac{KL({Q}||{P})}{2}}}{2} \le \frac{\sqrt{KL({P}||{Q}) + KL({Q}||{P})}}{2}.
% \end{align*}
%   \begin{align*}
%     & \;\textrm{Error}(\tilde{P}^{(1)}, \tilde{P}^{(0)}) = \; 0.5 - 0.5 \cdot {TV}(\tilde{P}^{(1)}, \tilde{P}^{(0)}).
% \end{align*}
% \begin{align*}
%   & \; \arg \max_{\Sigma_1, \Sigma_0} \textrm{Error}(\tilde{P}^{(1)}, \tilde{P}^{(0)}) \\
%   =& \; \arg \min_{\Sigma_1, \Sigma_0} TV(\tilde{P}^{(1)},\; \tilde{P}^{(0)}) \\
%   =& \; \arg \min_{\Sigma_1, \Sigma_0} TV(\mathcal{N}(g^{(1)}, \Sigma_{+} + \Sigma_{1}),\; \mathcal{N}(g^{(0)}, \Sigma_{-} + \Sigma_{0}))
% \end{align*}
% Let the minimal sum of KL be denoted as $\textrm{sumKL}^*$. Then we know for our minimizing solution $(\widetilde{\Sigma}_1, \; \widetilde{\Sigma}_0)$, we have $\textrm{Error}_{0.5}(\tilde{P}^{(1)}, \tilde{P}^{(0)}) \ge& \; \frac{1}{2} - \frac{\sqrt{\textrm{sumKL}^*}}{4}$. To maximize the error probability，we need minimize $\textrm{sumKL}^*$. 
In an extreme case, we can add infinitely large noise for both negative and positive gradients, then sumKL$^*$ will be $0$ and the error probability will be $0.5$ which is equivalent to a random guess. However, stochastic gradient descent  cannot converge under infinitely large gradient noise, so it is necessary to control the variance of the additive noise. We thus introduce the noise power constraint: $p \cdot \tr(\Cov[\noisevec^{(1)}]) + (1-p)\cdot\tr(\Cov[\noisevec^{(0)}]) \le \; P$, where $p$ is the fraction of positive examples (known to the active party), $\tr(\Cov[\noisevec^{(i)}])$ denotes the trace of the covariance matrix of the random noise vector $\noisevec^{(i)}$, and the power constraint $P$ is a tunable hyper-parameter to control the level of noise. Now the constrained optimization problem can be written as follows:
\begin{align}
    &\min_{\widetilde{P}^{(1)}, \widetilde{P}^{(0)}} \KL{\widetilde{P}^{(1)}}{\widetilde{P}^{(0)}} + \KL{\widetilde{P}^{(0)}}{\widetilde{P}^{(1)}} \label{eq:protection_objective_constrained} \\
&\quad \textrm{s.t.} \quad p \cdot \tr(\Cov[\noisevec^{(1)}]) + (1-p)\cdot\tr(\Cov[\noisevec^{(0)}]) \le \; P. \nonumber 
\end{align}
% The larger $P$ value, the larger the search space the algorithm has. If the $P$ is positive infinity, then the $\textrm{sumKL}^*$ will become $0$. The labeling function will work like a random guess. A larger $P$ value can introduce more more noise to the gradients of instances, and it can hurt the model's performance more easily.

\paragraph{Optimizing the objective.}
\label{sec: optimization}
%  we now have
%   \begin{align*}
%     \min_{\Sigma_1, \Sigma_0 \in \Sym^{d \times d}_{+}} & KL（{\mathcal{N}(g^{(1)}, \red{vI} + \Sigma_{1})} || {\mathcal{N}(g^{(0)}, \red{uI} + \Sigma_{0})}）\\
%   & \qquad + KL（{\mathcal{N}(g^{(0)}, \red{uI} + \Sigma_{0})} || {\mathcal{N}(g^{(0)}, \red{vI} + \Sigma_{0})}） \\
%   \\
%     \textrm{s.t.} \qquad & p \cdot \tr(\Sigma_1) + (1-p)\cdot \tr(\Sigma_0) \le \; P
%   \end{align*}
We introduce some assumptions in order to solve the optimization problem. We assume that the distribution of gradients (across samples) are Gaussian: $g^{(1)} \sim \mathcal{N}(\bar{g}^{(1)}, uI_{d \times d})$ and $g^{(0)} \sim \mathcal{N}(\bar{g}^{(0)}, vI_{d \times d})$. Let $\Delta g = \bar{g}^{(1)} - \bar{g}^{(0)}$ denote the difference of the two mean vectors. Additionally, we consider Gaussian additive noise: $\noisevec^{(1)} \sim \mathcal{N}(0, \Sigma_1)$ and $\noisevec^{(0)} \sim \mathcal{N}(0, \Sigma_0)$ where
the covariance matrices commute: $\Sigma_1 \Sigma_0 = \Sigma_0 \Sigma_1$. Then we have the following theorem.
\begin{theorem}
\label{thm:optimal_solution}
    The optimal $\Sigma_1^*$ and $\Sigma_0^*$ to \eqref{eq:protection_objective_constrained} have the form
    \begin{align*}
        &\Sigma_1^* = \frac{\Lam{1}{1} - \Lam{2}{1}}{\norm{\Delta g}_2^2} (\Delta g)(\Delta g)^{\top} + \Lam{2}{1}I_d, \qquad \\
        &\Sigma_0^* = \frac{\Lam{1}{0} - \Lam{2}{0}}{\norm{\Delta g}_2^2} (\Delta g)(\Delta g)^{\top} + \Lam{2}{0}I_d,
    \end{align*}
    where $(\Lam{1}{0}, \Lam{2}{0}, \Lam{1}{1}, \Lam{2}{1})$ is the solution to the following 4-variable optimization problem:
    \begin{align*}
    &\min_{\lambda_1^{(0)}, \lambda_1^{(1)}, \lambda_2^{(0)}, \lambda_2^{(1)}} \; (d-1) \frac{\lambda_2^{(0)} + u}{\lambda_2^{(1)} + v} + (d-1) \frac{\lambda_2^{(1)} + v}{\lambda_2^{(0)} + u} 
    \\&+ \frac{\lambda_1^{(0)} + u + \|\Delta g\|_2^2}{\lambda_1^{(1)} + v} + \frac{ \lambda_1^{(1)} + v + \|\Delta g\|_2^2}{\lambda_1^{(0)} + u}\\
   \textrm{s.t.} & \quad p \lambda_1^{(1)} + p(d-1) \lambda_2^{(1)}+ (1-p) \lambda_1^{(0)}\\
   &+ (1-p)(d-1)(\lambda_2^{(0)}) \le \; P,\nonumber \\
    & \, \lambda_1^{(1)} \le \; 0,\quad - \lambda_1^{(0)} \le \; 0, \quad - \lambda_2^{(1)} \le \; 0, \quad - \lambda_2^{(0)} \le \; 0, \nonumber \\
    & \, \lambda_2^{(1)} - \lambda_1^{(1)} \le \; 0, \qquad \lambda_2^{(0)} - \lambda_1^{(0)} \le \; 0 \nonumber.
  \end{align*}
  %\vspace{-0.35in}
\end{theorem}
%   Suppose $\Sigma_{-} \approx uI$ and $\Sigma_{+} \approx vI$, through simplification, we can convert this problem into a $\mathbf{4}$ variable optimization problem instead of $O(d^2)$. ($c \coloneqq \norm{g^{(1)} - g^{(0)}}^2_2$)
  
%   \begin{align*}
%     \min_{\lambda_1^{(0)}, \lambda_1^{(1)}, \lambda_2^{(0)}, \lambda_2^{(1)}}& \; (d-1) \frac{\lambda_2^{(0)} + u}{\lambda_2^{(1)} + v} + (d-1) \frac{\lambda_2^{(1)} + v}{\lambda_2^{(0)} + u} + \frac{\lambda_1^{(0)} + u + c}{\lambda_1^{(1)} + v} + \frac{ \lambda_1^{(1)} + v + c}{\lambda_1^{(0)} + u}\\
%   \textrm{s.t.} & \nonumber \\
%     & p \lambda_1^{(1)} + p(d-1) \lambda_2^{(1)}+ (1-p) \lambda_1^{(0)}+ (1-p)(d-1)(\lambda_2^{(0)}) \le \; P \nonumber \\
%     & \threequad - \lambda_1^{(1)} \le \; 0,\quad - \lambda_1^{(0)} \le \; 0, \quad - \lambda_2^{(1)} \le \; 0, \quad - \lambda_2^{(0)} \le \; 0 \nonumber \\
%     & \tenquad \lambda_2^{(1)} - \lambda_1^{(1)} \le \; 0 \nonumber \\
%     & \tenquad \lambda_2^{(0)} - \lambda_1^{(0)} \le \; 0 \nonumber.
%   \end{align*}
The optimal noise consists of two independent components: one random component lies along the direction of the difference between the positive and negative gradient mean vectors $\Delta g$ (whose covariance matrix is proportional to  $\Delta g \Delta g^{\top}$); the other component is sampled from an isotropic Gaussian. $\Sigma_1^*$ and $\Sigma_0^*$ have different mixture coefficients of these two components. 
%The detailed derivation of the theorem can be found in the next section. 
The detailed derivation of Theorem \ref{thm:optimal_solution} can be found in the appendix.


%   Because there is a linear equation that links the three variables together, we can use an optimization algorithm similar to \textbf{Sequential Minimal Optimization (SMO)} as used in SVM to solve this problem. Here every time we fix one of the three variables, then by the linear relationship between the rest two variables we can optimize the function to optimality (either analytically or numerically). Alternating between different fixed variable gives us an iterative algorithm to monotonically decrease the objective. %Two observations are important about this problem: \textbf{1)} the problem is not convex. Take $u=v=g=1$, the component $\frac{x + u + g}{y + v} + \frac{y + v + g}{x + u}$ at $x=0.01, y=10$ has its hessian with a negative determinant. \textbf{2)} However, when we fix one of the three variables, and only look at the restricted line segment, the function is in fact convex.
 
%  \subsection{Protection through Randomness}
%  \OS{Don't need to talk about implementation details in the main paper}
% With solution to  $(\Lam{1}{0}, \Lam{2}{0}, \Lam{1}{1}, \Lam{2}{1})$, the covariance matrix $\Sigma_0^*$ and $\Sigma_1^*$ of noise to be added to the negative and positive instances respectively are:

% \begin{align*}
%     \Sigma_0^* =& \; Q^T \diag(\Lam{1}{0}, \Lam{2}{0} \ldots, \Lam{2}{0}) Q \\
%     =& \; \frac{\Lam{1}{0} - \Lam{2}{0}}{\norm{g^{(1)} - g^{(0)}}_2^2} (g^{(1)} - g^{(0)})(g^{(1)} - g^{(0)})^T + Q^T \diag(\Lam{2}{0}, \Lam{2}{0} \ldots, \Lam{2}{0}) Q\\
%     =& \; \frac{\Lam{1}{0} - \Lam{2}{0}}{\norm{g^{(1)} - g^{(0)}}_2^2} (g^{(1)} - g^{(0)})(g^{(1)} - g^{(0)})^T + \Lam{2}{0}I_d
% \end{align*}

% We know that the distribution of $X \sim \mathcal{N}(\mathbf{0}, \Sigma_0^*) \eqd Y + Z$, where 
% \begin{align*}
%     Y \sim& \; \mathcal{N}(\mathbf{0}, \frac{\Lam{1}{0} - \Lam{2}{0}}{\norm{g^{(1)} - g^{(0)}}_2^2} (g^{(1)} - g^{(0)})(g^{(1)} - g^{(0)})^T), \\
%     Z \sim& \; \mathcal{N}(\mathbf{0}, \Lam{2}{0}I_d).
% \end{align*}

% For $W = \sigma \epsilon g$, where $\epsilon \sim \mathcal{N}(0, 1)$. Then 
% \begin{align*}
%     \textrm{Cov}(W) =& \E[(W-\E[W])(W-\E[W])^T] \\
%     =& \E[\sigma^2 \epsilo\noisevec^2 gg^T] \\
%     =& \sigma^2\E[\epsilo\noisevec^2] gg^T \\
%     =& \sigma^2 gg^T
% \end{align*}

% As a result, we can construct $Y$ as 
% \begin{align*}
%     Y = \epsilon \paren{\sqrt{\Lam{1}{0} - \Lam{2}{0}}} \frac{g^{(1)} - g^{(0)}}{\norm{g^{(1)} - g^{(0)}}_2}, \; \epsilon \sim \mathcal{N}(0, 1)
% \end{align*}

% And we can construct $Z$ as

% \begin{align*}
%     Z = \sqrt{\Lam{2}{0}}\mathbf{\epsilon}, \; \mathbf{\epsilon} \sim \mathcal{N}(\mathbf{0}, I_d)
% \end{align*}

% Similarly, for positive instances, we have

% \begin{align*}
%     \Sigma_1^* =& \; Q^T \diag(\Lam{1}{1}, \Lam{2}{1}, \ldots, \Lam{2}{1}) Q \\
%     =& \; \frac{\Lam{1}{1} - \Lam{2}{1}}{\norm{g^{(1)} - g^{(0)}}_2^2} (g^{(1)} - g^{(0)})(g^{(1)} - g^{(0)})^T + \Lam{2}{1}I_d
% \end{align*}

% \WH{Can we add comparison with white Gaussian noise and perpendicular noise here?}

% \subsection{Approximate theoretical guarantees}

% \WH{We can formally write a theorem for our theoretical guarantee}

In practice, we can estimate $\bar{g}^{(1)}$, $\bar{g}^{(0)}$, $u$, and $v$ using maximum likelihood estimation with the mini-batch's $g$ of the current communication round. With these parameters computed, the 4-variable optimization problem can be easily solved by an alternating optimization algorithm similar to \textit{Sequential Minimal Optimization} (SMO) used in SVM \cite{platt1998sequential}. We note that by varying $P$ we can achieve different trade-offs between label privacy and model performance. Larger $P$ will give smaller $\textrm{sumKL}^*$, and therefore smaller leak AUC, but worse model performance. To achieve a lower bound $L$ of the worst-case detection error, we simply require that the optimal sumKL value to be  $\textrm{sumKL}^* \le (2 - 4L)^2$ by the aforementioned upper bound of total variation distance. We could achieve this by keeping on increasing the value of $P$ used in the power constraint until the corresponding $\textrm{sumKL}^*$ satisfies this requirement.



==> Backup/tex/introduction.tex <==
With the increasing concerns on data security and user privacy in machine learning, \textit{federated learning} (FL)~\citep{mcmahan2017communication} becomes a promising solution to these challenges. Based on how sensitive data are distributed among various parties, FL can be classified into different categories~\citep{yang2019federated}, notable among which are \textit{vertical FL} and \textit{horizontal FL}. %: horizontal FL, Vertical FL, and Federated Transfer Learning. 
Different from horizontal FL where the data are partitioned by examples, vertical FL assumes that the data are partitioned by different features (including labels). %Vertical FL happens in a classic online advertising setting.
%Compared to horizontal FL which are starting to find real-world large-scale applications, vertical FL already has many possible use cases (especially in online advertising) for years. \WH{Is there any citations? If so, add them here. If not, we can delete this sentence and just say that we focus on vertical setting in this paper}
%\JK{it's better to introduce split learning here} \OS{Split learning considers how the model does inference and training; vertical FL concerns how the data is split. Vertical FL needs split learning but horizontal FL could also use split learning}
A typical example of vertical FL is when an online media platform $A$ displays advertisements of an ecommerce company $B$ to its users and charges $B$ for each \textit{conversion} (e.g., user clicking the ad and buying the product). %(when a user clicks on an ad and subsequently purchases the corresponding product from $B$). 
In this case, both parties have different features for the same set of users: party $A$ has features on users' media viewing records and party $B$ has the users' product browsing records and conversion labels. The conversion labels are not available to party $A$ because users' buying processes happen entirely on party $B$'s website/mobile app.
%once a user clicks on an ad displayed on $A$'s platform, he/she leaves the platform and is directed to $B$'s website/mobile app. Thus whether a purchase is made is not known to $A$. %\WH{This paragraph can be presented better with a figure. I remembered Jiankai has a figure on vertical v.s. horizontal in one of his presentations}%On the other hand, the advertiser knows users' purchasing history but do not know what users have browsed other than its own ad, e.g. what news stories/tweets or ads from other advertisers the user has shown interest in.

If both parties want to train a deep learning model jointly to predict the conversion rate based on feature-partitioned data, they could sign legal agreements to allow them to share the data with each other.
However, due to privacy and business concerns, recently companies  are unwilling to share their data with  other parties.  
%\red{Following the same setting as (~\citep{cheng2019secureboost}), we consider the party which holds the label as active party, and the other as the passive party.} 
\textit{Split learning}~\citep{gupta2018distributed,vepakomma2018split} enables the joint training of deep learning models without sharing sensitive data by splitting the execution of a deep learning model between the parties on a layer-wise basis. In vanilla split learning, the party without labels (called the \textit{passive party}) sends the computation results of the intermediate layer (called the \textit{cut layer}) rather than the raw data to the party with labels (called \textit{active party}). The active party then completes the rest of the forward step computation, computes the gradients based on the labels, and sends the gradients with respect to the cut layer back to the passive party. The passive party then completes the back propagation with the gradients of the cut layer using chain rule. 
%\WH{Our paper is based on split learning, so I think it would be better to introduce split learning earlier.}

At first glance, the process of split learning seems private because only the intermediates computation results of the cut layer,
rather than raw features or labels, are communicated between the two parties. 
%One could naively believe that the raw data cannot be recovered from these communications. 
%In a typical training process of the Vertical FL, the passive party sends embeddings to the active party, and the active party computes the corresponding gradients w.r.t the loss based on the label information and sends the gradients back to the passive party.
However, such ``gradient sharing'' scheme has been shown to be vulnerable in the setting of horizontal FL: 
in a recent work of \citet{zhu2019dlg},
it is shown that  the central server could recover raw features and labels of a device using model parameters and gradients shared by that device.
% recently \citeauthor{zhu2019dlg} (\citeyear{zhu2019dlg}) demonstrated that in \textbf{horizontal} FL setting, the central server could recover raw features and labels of a device using model parameters and gradients shared by that device.
%\WH{DLG and iDLG can be discussed in related work, we can directly introduce our main contributions} \JK{DLG and iDLG shows that sharing gradients can leak information. I think it's necessary to keep this description here. Otherwise, readers may think that   sharing gradients can leak information is our novel observation.}
We wonder whether the raw data (specifically the labels from the active party) can also be leaked by sharing gradients of the cut layer in the \textbf{split learning} (vertical FL) setting. 

In this work, we first identify a simple but accurate method that uses the norm of the communicated gradients from the active party to uncover the labels in imbalanced datasets. 
%Moreover, we propose a theoretically justified protection technique which strategically perturbs the gradient randomly before communication and can protect a wide class of label-uncovering methods including the proposed norm-based method. 
We then discuss several protection techniques to mitigate this issue.  Among them, we have designed a principled approach that directly maximizes the worst-case error of label detection. This theoretically justified technique strategically perturbs the gradient randomly before communication. We experimentally demonstrate the effectiveness and competitiveness of the proposed protection method compared to other baselines. 
%The rest of this paper is organized as follows. After reviewing some related works in Section~\ref{sec:related-work}, we formally describe the split learning formulation on binary classification and introduce the norm-based label attack method in Section~\ref{sec:framework}. Then we introduce the theoretically justified protection technique in Section~\ref{sec:protection}. Experiment results demonstrating the advantages of our proposed method can be found in Section~\ref{sec:experiment}.

\begin{comment}
In this paper, we first propose a more general approach than iDLG to extract the ground-truth labels from the shared gradients w.r.t hidden layers of any NN with cross-entropy loss over one-hot labels. By deviation, we demonstrated that the gradient norm of positive instance are larger than the negative ones'. With this rule, we can uncover the label of instances by ranking the corresponding gradient norms in a mini-batch and select the top ones as the positive instances. 

The norm attack described above puts a server challenge to the current vertical FL and some split learning settings. We then propose to use gradient perturbation strategy to prevent label leakage. The amount of the perturbation is determined by minimizing the symmetrized KL divergence between perturbated gradients of positive and negative instances. To avoid add unlimited noise to the gradients and make the model converge, some constraints are added to the minimization problem. An approximate theoretical guarantee is achieved for this protection strategy. Extensive experiments demonstrated that we can achieve a reasonable trade-off between model performance and protection quality.
\end{comment}


==> Backup/tex/live_experiments.tex <==

% \vspace{-0.125in}
\subsection{Experiments on Real Production Dataset}
\label{sec:live_experiments}

While the results on public dataset shed light upon the behaviors of the proposed protection methods, it's more important to understand if they could have reasonable trade-off between privacy and utility for conversion rate (CVR) prediction tasks in industrial environments. %Our experimental platform is one of the largest in the industry with hundreds of millions of users. 
Our experimental platform is an open sourced federated learning framework Fedlearner\footnote{\url{https://github.com/bytedance/fedlearner}} that enables joint modeling of data distributed between industrial parties with hundreds of millions of users. In our system, the passive party is an online media platform and it displays advertisements for an ecommerce company (the active party) to its users. %The passive party charges the active party for each conversion. %Both parties have different features for the same set of users: the passive party has features on users' media viewing records and the active party has the users' product browsing records and conversion labels. 
Users' buying processes happen entirely on the active party's website/mobile app. And the active party would like to protect their conversion labels from leakage. We reported different protection methods' daily averaged performance of utility and privacy with data ranging from January to February 2020 (about $42.56$ million records of users' conversion) \footnote{We follow the stream learning protocol to train the model and the batch size is set as $1,024$.} in Figure~\ref{fig:live_experiments}:

% \vspace{-0.15in}
% \begin{itemize}[leftmargin=0.1in,noitemsep]

1) \maxnorm{} and iso\_1.0 can achieve similar utility.\footnote{Here iso\_1.0 indicates the parameter of white Gaussian $s$ is set as $1.0$ and others are similarly defined.} However, iso\_1.0 has the worst leak AUC on both norm and hint attack among all protection methods (excluding the baseline: \nonoise). {iso\_2.0} adds more isotropic Gaussian noise than {iso\_1.0} and as a result, { iso\_2.0} can achieve better privacy than { iso\_1.0}. It is worth mentioning that {iso\_2.0} can have better hint attack protection than {\maxnorm}. Unfortunately, {iso\_2.0} achieves the worst utility among all the methods. Additionally, most of the times, variants of Marvell (sumKL\_0.1 and sumKL\_0.25)\footnote{Here sumKL\_0.1 indicates the optimization objective of $\textrm{sumKL}^*$ in Eq.~\ref{eq:protection_objective_sumKL} is set as $0.1$. Others are similarly defined.} can have better leak AUC on norm and hint attack than {iso\_2.0}. We can conclude that using isotropic Gaussian noise is the most difficult one to achieve the reasonable trade-off between utility and privacy among all the protection methods.

2) \marvell \ achieves the best overall privacy on preventing the norm and hint attack. Compared with the baseline {no\_noise} without any protection, {sumKL\_0.25} and {sumKL\_0.1} drop the performance AUC about $1.53\%$, and $1.80\%$ as a trade-off respectively. As {\maxnorm} is designed to prevent norm attack, it achieves similar norm attack AUC with {sumKL\_0.25} with a performance drop about $1.02\%$ comparing with {no\_noise}. However, {\maxnorm} becomes less effective than {sumKL\_0.25} when dealing with hint attack. Overall, these experimental results show that \marvell{} performs well in the industrial environments. %It's possible that some unknown gradient distribution based attack methods can breach {\maxnorm} since it has no theoretical guarantee. Unlike \maxnorm, Marvell is a theoretically principled method to determine the best perturbation added to the gradients. It can reduce the probability of label leakage against unknown attacks.
% \end{itemize}

==> Backup/tex/max_norm_alignment.tex <==
% \subsubsection{Max norm alignment to prevent label leakage}
% \label{sec:max_norm_alignment}

We now introduce an improved way to add Gaussian noise by making the expected norm of the positive and negative gradients in a mini-batch equal (un-distinguishable). The key question is how to determine the standard deviation of the Gaussian noise with zero mean added to each gradient. For simplicity, we can align all the instances to have the same expected norm with the maximum gradient norm among the mini-batch. Hence, we name this heuristic protection method as {\tt max\_norm}. %It's worth mentioning that the instance which has the maximum norm is a positive one. 
Suppose that instance $i$ in a mini-batch has the maximum gradient norm and its corresponding gradient is $g_i$. For arbitrary $j$,
let instance $j$'s gradient be $g_j$. 
The noise we add is $\eta_j\cdot g_j$, where $\eta_j\sim \mathcal{N}(0,\sigma_j^2)$ and $\sigma_j$ is the standard deviation to be determined. 
The perturbed gradient of $g_j$ is $g'_j = g_j(1+\eta_j)$,
and we require (the square of) the expected norm of ${g'_j}^2$ to be aligned to that of $g_i$,
% The standard deviation $\sigma_j$ of the Gaussian noise added to perturbate the gradient $g_j$ is calculated by making their expected norm equal, 
then we have: $$\|g_i\|_2^2=\mathbb{E}(||g_j||^2(1 + \eta_j)^2) =  ||g_j||^2(1 + \sigma_j^2).$$ Hence $\sigma_j = \sqrt{{||g_i||^2}/{||g_j||^2} - 1}$. As designed, \maxnorm \ can prevent the norm attack very well (more details can be seen in the experimental section). The advantage of \maxnorm \ is that it has no parameter to tune. Unfortunately, it does not have a theoretical guarantee of the trade-off between model utility and privacy and it may be breached by some unknown attacks. 

% \begin{equation}
% \begin{split}
% E(||g_i||^2) = E(||g_j||^2(1 + 2 \sigma_j + \sigma_j^2)) \\
% E(||g_i||^2) = E(||g_j||^2(1 + \sigma_j^2)) \\
% \sigma_j^2 = \frac{||g_i||^2}{||g_j||^2} - 1   \\
% \sigma_j = \sqrt{\frac{||g_i||^2}{||g_j||^2} - 1} \\
% \end{split}
% \end{equation}

% The corresponding algorithm is described as Algorithm~\ref{alg:max_norm}.

% \begin{algorithm}[H]
% \DontPrintSemicolon
%   \KwInput{$\mathbf{g}$: gradient sending back to the passive party; $n$ by $d$ where $n$ is the batch size, $d$ is the number embedding dimension. \;}
%   \KwOutput{$\mathbf{g'}$: perturbated gradient with Gaussian noise}
%     compute $max\_norm$ =  max($||\mathbf{g}_i||^2$),  $\forall i \in [1, n]$ \\
%  \For{i \leftarrow 1 \ to \ n}    
%         { \tcc{compute the standard deviation of the Gaussian noise}
%         $\sigma_i = \sqrt{max(\frac{||max\_norm||^2}{||\mathbf{g}_i^2||} - 1, 0)}$ \\
%         $noise_i \sim \mathcal{N}(0,\,\sigma_i^{2})$ \tcp*{generate the zero mean Gaussian noise}\\
%         $\mathbf{g'}_i = \mathbf{g}_i (1 + noise_i)$ \tcp*{add the generated noise to the gradient} \\
%         }
%  \textbf{Return} $\mathbf{g'}$
% \caption{Max Norm Alignment to Preventing Label Leakage}
% \label{alg:max_norm}
% \end{algorithm}

% The disadvantage of this algorithm is that it does not have a theoretical guarantee.

==> Backup/tex/norm_attack.tex <==
%In this section, we provide a strategy to extract ground-truth labels named as norm attack in the binary classification scenario. %The neural network %as illustrated in Figure~\ref{fig:illustration_NN} 
%is trained with cross-entropy loss. 
%The model training process is illustrated in Table ~\ref{tab:model_training}, where $\mathbf{X}$ is the input datum, $\bm{f}$ and $\bm{h}$ are networks of the passive and active party respectively, $L$ is the cross-entropy loss, $l$ is the output logit, $\tilde{p_1}$ is the corresponding predicted probability of being a positive label, and $y$ is the ground-truth label. %: $l(\mathbf{x}, c) = -log\frac{e^{y_c}}{\sum_j e^{y_j}}$, where $\mathbf{x}$ is the input datum, $c$ is the corresponding ground-truth label, $\mathbf{y} = [y_1 , y_2 , ...]$ is the outputs (logits), and $y_i$ denotes the score (confidence) predicted for the $i$-th class.
\label{sec:norm-attack}
From the expression of $g$, we see that the norm of the communicated gradient is $\norm{g}_2 = \abs{\widetilde{p}_1 - y} \cdot \norm{\nabla_a h(a) \vert_{a=\bm{f}(X)}}_2$. {This is always a linear function of $\abs{\widetilde{p}_1 - y}$, due to the linearity of back-propagation.} We identify two following observations for $\abs{\widetilde{p}_1 - y}$ and $\norm{\nabla_a h(a) \vert_{a=\bm{f}(X)}}_2$ which hold true for a wide range of real-world learning problems. Based on these observations, we propose a method to uncover the label $y$ by using the gradient norm $\norm{g}_2$. %\vspace{-0.15in}

\begin{itemize}[leftmargin=*]%[leftmargin=0.2in,noitemsep]
    \item Observation 1: Almost throughout the entire training, the model tends to be \textbf{less confident} about a positive example being positive \textbf{than} a negative example being negative.
    In other words, the confidence gap $1 - \widetilde{p}_1$ of a positive example ($y=1$) is typically larger than the confidence gap $ 1 - \widetilde{p}_0 = \widetilde{p}_1$ of a negative example ($y=0$). Thus the value of $|\widetilde{p}_1 - y|$ is typically higher for positive examples than that of the negative examples (Figure~\ref{fig:dist}.(a)).
    %In other words, $ 1 - \widetilde{p}_1$ of a positive example is typically greater than $\widetilde{p}_1$ of a negative example (Figure~\ref{fig:dist}.(a)). Thus the value of $|\widetilde{p}_1 - y|$ is typically higher for positive examples than that of the negative examples.
    This observation is generally true for problems like advertising conversion prediction and disease prediction, where there is inherently more ambiguity for the positive class than the negative. For example, in the advertising conversion problem, uninterested users of a product will never click on its ad and convert, but those interested, even after clicking on the ad, might make the purchase for only a fraction of the time depending on whether they at the moment have the time or money to execute the purchase. 
    \item Observation 2: Almost throughout the training, the norm of the gradient vector { $\norm{\nabla_a h(a) \vert_{a=\bm{f}(X)}}_2$} is on the \textbf{same} order of magnitude for both the positive and negative examples (Figure~\ref{fig:dist}.(b)). This is natural because $\nabla_a h(a) \vert_{a=\bm{f}(X)}$ is not a function of $y$.
\end{itemize}

As a consequence of these two observations, the gradient norm $\norm{g}_2$ of the positive instances are generally \textbf{larger than} that of the negative ones (Figure~\ref{fig:dist}.(c)). Thus, $\norm{g}_2$  is a very strong predictor of the unseen label $y$. We quantitatively measure how well $\norm{g}_2$ can predict $y$ by the AUC of the ROC curve when using $\norm{g}_2$ as a predictor of $y$. 
We call this value \textit{leak AUC}. This value can be estimated at every gradient update iteration using the minibatch of examples used in that batch. Higher leak AUC means the label is leaked more consistently by the communicated gradient $g$. In the Criteo dataset experiment in Figure~\ref{fig:dist}, the leak AUC for the four iterations presented are $0.9832$, $0.8862$, $0.9098$, $0.9229$, signaling generally a high level of label leakage throughout the model training.

\textit{Other Related Attacks.} We also observe that positive and negative instances have opposite gradient directions ($ \widetilde{p}_1 - 1 < 0$ for positive instances, and $\widetilde{p}_1 > 0$ for negative ones) {no matter whether the dataset is balanced or not}.
We can compute the pairwise cosine similarity for all instances in the mini-batch based on their corresponding gradients. We infer an instance as negative if its cosine similarity is dominated by positive values (due to the imbalance of data), otherwise it is positive. This attack is highly related with aforementioned norm attack and our protection methods are still effective for this attack. For the sake of space, we only report norm attack in this paper. 

%In Figure \ref{fig:dist} (a), we notice that the distribution of $\abs{\widetilde{p}_1 - y}$ of the positive examples is to the right of that of the negative examples (observation 1). In Figure \ref{fig:dist}(b), positive and negative examples's distribution of $\norm{\nabla_a h(a) \vert_{a=\bm{f}(X)}}_2$ are almost exactly matching (observation 2). As a result, positive examples' $\norm{g}_2$ is generally larger for positive examples.

%In addition, for many practical learning problems, (\textbf{Assumption}) the passive party, despite not having direct access to the label of every example in the batch, has a very good estimate of the fraction of positive examples in a random batch, e.g. the conversion rate of the entire user base for online advertising or the total fraction of the population developing a disease for disease prediction. As a result, by the two observations and this assumption, \textbf{simply ranking the communicated gradient according to their $2$-norm and taking only the top known fraction as positive with the rest as negative} will uncover almost $100\%$ of all the labels in a random batch \footnote{see Experiments for empirical confirmation}.
\begin{figure*}[t] 
   \vspace{-0.05in}
  \begin{minipage}[b]{0.31\linewidth}
  \centering
    \includegraphics[width=\linewidth]{figures/logit_grad_hist100-200-300-400.pdf}
    \vspace{-2.0em}
    \caption*{(a)}
  \end{minipage}
  \begin{minipage}[b]{0.31\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/h_grad_dist100-200-300-400.pdf}
    \vspace{-2.0em}
    \caption*{(b)}
    %\captionsetup[figure]{labelformat=empty}
  \end{minipage} 
  \begin{minipage}[b]{0.31\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/g_dist100-200-300-400.pdf}
    \vspace{-2.0em}
    \caption*{(c)}
  \end{minipage} 
  \vspace{-0.5em}
 \caption{We demonstrate these two observations and the consequence with a Wide \& Deep model \cite{cheng2016wide} trained on the Criteo dataset for click-through rate prediction (problem in online advertising similar to conversion prediction). Here the passive party $f$ includes the embedding layer and the first two layers of a four layer multi-layer perceptron (MLP) (the deep part); the active party includes the other two layers of the deep part together with the wide part of the model. Here the communicated gradient $g$ is of the middle cut layer in the deep part. We show the distribution of $\abs{\widetilde{p}_1 - y}$, $\norm{\nabla_a h(a) \vert_{a=\bm{f}(X)}}_2$, and $\norm{g}_2$ for both positive and negative examples after the first $100$, $200$, $300$, $400$ steps of stochastic gradient descent training in (a), (b), (c) respectively.}
 \label{fig:dist}
 \vspace{-0.2in}
\end{figure*}

% \WH{1. For the observation, is it possible to provide simple experiment results to support the observations here?}
% \WH{2. ``gradient of positive instances are much larger than negative ones' '' is a consequence of the two observations, or an independent observation?}
% \WH{3. Is this assumption necessary for the passive party?}
% \WH{4. Add experiment result in the end of this section?}
  
  %For every $(X, y)$ in the mini-batch, the exchanged gradient between both parties is $ g = \underbrace{(\widetilde{p}_1 - y)}_{\mbox{\scriptsize $\in$} \mathbb{R}}\nabla_a h(a) \bigg \vert_{a=\bm{f}(X)}$, where $||{\nabla_a h(a) \bigg \vert_{a=\bff(X)}}||_2$ has the same magnitude for examples with $y=0$ and $y=1$. The only difference is $\widetilde{p}_1 - y$. In a unbalanced dataset, such as online advertising and health related areas,  where positive instances are much less than the negative instances, for instances with $y = 1$, the predicted probability $\widetilde{p}_1 \ll 1$ and $|\widetilde{p}_1 - y| = |\widetilde{p}_1 - 1| \approx 1$. For negative instances ($y = 0$), we have $\widetilde{p}_1 \approx 0$ and $|\widetilde{p}_1 - y|= |\widetilde{p}_1 - 0| \approx 0$. Hence, the gradient norm of positive instances are much larger than the negative ones. With above observation, the adversary can rank all the instances in a mini-batch based on their gradient norms and select the top ones as the positive instances.
  
  
%   \begin{itemize}
%     \item if $y = 1$, then $\widetilde{p}_1 \ll 1$ $\implies$ $|\widetilde{p}_1 - y| = |\widetilde{p}_1 - 1| \approx 1$
%     \item if $y = 0$, then $\widetilde{p}_1 \approx 0$ $\implies$ $|\widetilde{p}_1 - y|= |\widetilde{p}_1 - 0| \approx 0$.
%   \end{itemize}
  
  % In a unbalanced dataset where positive instances are much less than the negative instances, the predicted probability $p_1$ will be much smaller than $p_0 = 1 - p_1$. Hence, the gradient norm of positive instances are much larger than the negative ones. It happens a lot in online advertising and health related areas. With above rule, we can rank all the instances in a mini-batch based on their gradient norms and select the top ones as the positive instances. %, as shown in Figure ~\ref{fig:g_norm}.

  
%   \begin{align*} g = \underbrace{(\widetilde{p}_1 - \red{y})}_{\mbox{\scriptsize $\in$} \mathbb{R}}\nabla_a h(a) \bigg \vert_{a=\bm{f}(X)}, \; \textrm{for every $(X, y)$ in the minibatch}.\end{align*}


% Then, the gradients of the loss w.r.t. each of the outputs is:

% \begin{equation*}
%     g_i = \frac{\partial {l(\mathbf{x}, c)}}{\partial{y}_i} = -\frac{\partial log (e^{y_c}) - \partial log (\sum_j e^{y_j})}{\partial y_i} \\
%     & = \begin{cases}
%     -1 + \frac{e^{y_i}}{\sum_j e^{y_j}} &\text{if $i = c$}\\
%     \frac{e^{y_i}}{\sum_j e^{y_j}} &\text{else}
%     \end{cases}
% \end{equation*}

% {\em iDLG} proposed by ~\cite{zhao2020idlg} identified the ground-truth label as the index of the output that has the negative gradient. However, this rule can only be applied to the logit layer. We now show how can we extract the ground-truth labels based on the shared gradients of the split layers.

% The gradient vector $\nabla{\mathbf{W}}_{L}^{i}$ w.r.t. the weights $\mathbf{W}_{L}^{i}$ connected to the $i$-th logit in the output layer can be
% written as:

% \begin{equation}
%     \nabla{\mathbf{W}_{L}^{i}} = \frac{\partial {l(\mathbf{x}, c)}}{\partial{y}_i} \cdot  \frac{\partial{y}_i}{\partial{\mathbf{W}_{L}^i}} = g_i \cdot \mathbf{a}_{L-1}
% \end{equation}

% \begin{figure*}
%     \includegraphics[width=0.95\textwidth]{figures/Label_Leakage_Illustration.pdf}
%     \caption{Illustration of the neural network: The passive party sends the embedding to the active party. The active party computes the gradient w.r.t the split layer and sends it to the passive party.}
%     \label{fig:illustration_NN}
% \end{figure*}

% \section{Inferring Label from Gradients Norm}


% Without loss of generality, given one instance in a setting of multi-class/label:


% \begin{equation}
%      p_i = \frac{e^{y_i}}{\sum_j e^{y_j}}
% \end{equation}

%  \begin{equation}
%      y_i = {\mathbf{W}_{L}^{i}}^T \mathbf{a}_{L-1} + b_{L}^{i}
%  \end{equation}
 
%  Suppose the network has $L$ layers. $\mathbf{y} = \mathbf{a}_L$ is the output layer activation. The corresponding weights matrix  which connected to the $i$-th logit in the output layer is $\mathbf{W}_{L}^{i}$. And $b_{L}^{i}$ is the bias parameter. We then have $p_i = \frac{e^{y_i}}{\sum_j e^{y_j}}$ and $y_i = {\mathbf{W}_{L}^{i}}^T \mathbf{a}_{L-1} + b_{L}^{i}$.

% \begin{equation}
%     \nabla{\mathbf{a}_{L-1}} = \sum_i \frac{ \partial {l(\mathbf{x}, c)}}{\partial{y}_i} \cdot  \frac{\partial{y}_i}{\partial{\mathbf{a}_{L-1}}} \\
    
%     = \sum_i g_i \cdot\mathbf{W}_{L}^{i} = (-1 + p_c) \mathbf{W}_{L}^{c} + \sum_{i, i \neq c} p_i \mathbf{W}_{L}^{i} 
    
% \end{equation}

% In a binary classification, the  positive instances' gradient w.r.t to the cross-entropy loss of the split layer:

% \begin{equation}
%     \nabla{\mathbf{a}_{L-1}^1} = (-1 + p_1)\mathbf{W}_{L}^{1} + p_0 \mathbf{W}_{L}^{0}
% \end{equation}

% Similarly, for negative instances, we have:

% \begin{equation}
%     \nabla{\mathbf{a}_{L-1}^0} = (-1 + p_0)\mathbf{W}_{L}^{0} + p_1 \mathbf{W}_{L}^{1}
% \end{equation}

% Since $p_0 + p_1 = 1$, for positive instance, we then have:

% \begin{equation}
%     \nabla{\mathbf{a}_{L-1}^1} = (-1 + p_1)\mathbf{W}_{L}^{1} + (1 - p_1) \mathbf{W}_{L}^{0} = (1-p_1)(\mathbf{W}_{L}^{0} - \mathbf{W}_{L}^{1})
% \end{equation}

% Similarly, for negative instance, we have:

% \begin{equation}
%     \nabla{\mathbf{a}_{L-1}^0} = (-1 + 1 - p_1)\mathbf{W}_{L}^{0} + p_1 \mathbf{W}_{L}^{1} = -p_1 (\mathbf{W}_{L}^{0} - \mathbf{W}_{L}^{1})
% \end{equation}

% Applicable to multi hidden layers. Binary labels. 

% The gradients of the shared $K$-th hidden layers:

% \begin{equation}
%     \nabla{\mathbf{a}_{K}} = \sum_i \frac{ \partial {l(\mathbf{x}, c)}}{\partial{y}_i} \cdot  \frac{\partial{y}_i}{\partial{\mathbf{a}_{K}}} = \sum_i g_i \cdot \frac{\partial{y}_i}{\partial{\mathbf{a}_{K}}} = g_0 \cdot \frac{\partial{y}_0}{\partial{\mathbf{a}_{K}}} + g_1 \cdot \frac{\partial{y}_1}{\partial{\mathbf{a}_{K}}}
% \end{equation}

% In a binary classification, we have $p_0 + p_1 = 1$, then we derive the gradients of positive instance:

% \begin{equation}
%     \nabla{\mathbf{a}_{K}^1}  = (1-p_1)(\frac{\partial{y}_0}{\partial{\mathbf{a}_{K}}} - \frac{\partial{y}_1}{\partial{\mathbf{a}_{K}}})
% \end{equation}

% Similarly, for negative instances, we have:

% \begin{equation}
%     \nabla{\mathbf{a}_{K}^0}  = -p_1 (\frac{\partial{y}_0}{\partial{\mathbf{a}_{K}}} - \frac{\partial{y}_1}{\partial{\mathbf{a}_{K}}})
% \end{equation}

% In a unbalanced dataset where positive instances are much less than the negative instances, the predicted probability $p_1$ will be much smaller than $p_0 = 1 - p_1$. Hence, the gradient norm of positive instances are much larger than the negative ones. It happens a lot in online advertising and health related areas. With above rule, we can rank all the instances in a mini-batch based on their gradient norms and select the top ones as the positive instances. %, as shown in Figure ~\ref{fig:g_norm}.

% \begin{figure*}
%     \includegraphics[width=0.95\textwidth]{figures/g_norm.pdf}
%     \caption{2-norm attack to extract ground-truth labels}
%     \label{fig:g_norm}
% \end{figure*}

==> Backup/tex/related_work.tex <==
% \red{~\cite{zhao2020idlg} then proposed iDLG to extract ground-truth labels by exploiting the relationship between the labels and the signs of the corresponding gradients w.r.t output layer (or the logits layer) of any Neural Network (NN) with cross-entropy loss over one-hot labels, which is the general case for classification ~\citep{lyu2020threats}.} The limitation of this procedure is that it can not leverage above relationship and steal the ground-truth labels from the shared gradients w.r.t the hidden layers.
% \blue{talk about threats in FL paper}
\label{sec:related-work}
\textbf{Uncovering the raw data}. Even though raw data are not shared across different parties in federated learning, they are still not secure when gradients and model parameters are shared among different parties. In the horizontal FL setting, \citet{zhu2019dlg} showed that an honest-but-curious server can uncover the raw features and labels of a participating device by knowing the model architecture, parameters, and the communicated gradient of the loss on the device's data. Building upon the techniques in \citet{zhu2019dlg}, \citet{zhao2020idlg} showed that the ground truth label of an example can be extracted by exploiting the relationship between the directions of the gradients of the weights connected to the logits of different classes. In this work, we study a different setting in FL --- the two-party split learning setting for vertical FL~\cite{yang2019federated}, where no parties have access to the model architecture or model parameters on the other party's side. We show one can recover the ground-truth labels (not the raw input features \cite{vepakomma2019reducing}) by using magnitude ($2$-norm) instead of the direction of the gradients.

%\textbf{Privacy protection methods in FL}. Various methods have been proposed to protect the communicated messages among parties in FL. These methods can be broadly classified into three categories: \textbf{1)} cryptography-based methods such as \textit{Secure Multi-party Computation} \cite{agrawal2019quotient, du2004privacy, bonawitz2017practical, nikolaenko2013privacy} and \textit{homomorphic encryption} \cite{aono2017privacy, sathya2018review}; \textbf{2)} system-based methods such as \textit{Trusted Executation Environments} \cite{subramanyan2017formal, tramer2018slalom}; \textbf{3)} perturbation methods such as randomly perturbation of communicated message \cite{abadi2016deep, mcmahan2017learning}, reducing message's data-precision, compressing and sparsifying the message \cite{zhu2019dlg}, etc. Many statistical methods try to protect the privacy of each example / each device's dataset in horizontal FL setting when \textit{aggregated} \OS{This is not ture. In horizontal FL, each device is one ``record'', so there is no aggregation} information are shared among parties~\cite{abadi2016deep, geyer2017differentially, mcmahan2018general, mcmahan2017learning, bhowmick2018protection, thakkar2019differentially, pichapati2019adaclip, Rajkumar2012DP}. In this setting, \textit{differential privacy} \cite{DPDwork2006, dwork2014algorithmic} is widely used  to quantitatively ensure the security level of a protection method on \textbf{individual} records. The protection method proposed in this work belongs to the third category. However, we aim to protect the labels when \textit{non-aggregated} information are shared among parties, which brings more challenges.

\textbf{Privacy protection methods.} Because sharing intermediate computation results (model parameters, representations, gradients) might leak the raw data, FL communications will need to proceed in a privacy-preserving manner. There are generally three classes of approaches to communicate in a privacy-preserving manner: \textbf{1)} cryptography-based methods such as \textit{Secure Multi-party Computation} \cite{ du2004privacy,nikolaenko2013privacy, bonawitz2017practical,agrawal2019quotient} and \textit{homomorphic encryption}\cite{aono2017privacy, sathya2018review}; \textbf{2)} system-based methods such as \textit{Trusted Execution Environments} \cite{subramanyan2017formal, tramer2018slalom}; \textbf{3)} perturbation methods such as randomly perturbing the communicated message \cite{abadi2016deep, mcmahan2017learning}, shuffling the messages \cite{erlingsson2019amplification, cheu2019distributed}, reducing message's data-precision, compressing and sparsifying the message \cite{zhu2019dlg}, etc. Our work belongs to the third category where we add random perturbations to the gradients before communication to protect the labels. Many of the randomness-based privacy protection methods was proposed in the domain of horizontal FL where the aim is to protect the privacy of each example/ each device's dataset \cite{abadi2016deep, geyer2017differentially, mcmahan2018general,
mcmahan2017learning, bhowmick2018protection, thakkar2019differentially, pichapati2019adaclip, Rajkumar2012DP}. In this case, \textit{Differential privacy} (DP) \cite{DPDwork2006, dwork2014algorithmic} was used to quantitatively measure the proposed random mechanisms' ability to protect the privacy of any individual records.
To the best of our knowledge \cite{lyu2020threats}, in this paper, we introduce the first several randomness-based techniques to protect the active party's label privacy with the goal of maximizing detection error during split learning in vertical FL. 
% {\tt To discuss: Unlike the record-level privacy considered in DP, we consider protecting the \textbf{entire} training set's label information as a whole -- our approach reduces the percentage of the training set whose label information is leaked. We recognize that protecting each individual example's label information is also important and we leave it as future work. We note here that gradient-based label leakage occurs as long as the passive party gets access to the real gradients, regardless of the cryptographic scheme used in the learning protocol. Actually, if the passive party has prior knowledge on the distribution of the encrypted gradients, similar label leakage also occurs. 
% Though, due to the limits of the computation power of the passive learner, the label leakage under encryption might not be able to be exploited.
% %It might be more challenging to design protection with the presence of cryptosystem. 
% }

%only consider protecting the \textbf{entire} training set's label information as a whole -- our approach reduces the percentage of the training set whose label information is leaked but not focuses on giving a universal probability guarantee for not leaking any specific record's label information individually. We recognize that protecting each individual example's label information is also important and we leave it as future work.

%Recent study showed that direct sharing gradients might leak private information ~\citep{zhu2019dlg}. ~\citep{zhao2020idlg} \WH{do not start a sentence with an unnamed citation} then proposed iDLG to extract ground-truth labels by exploiting the relationship between the labels and the signs of the corresponding gradients w.r.t output layer (or the logits layer) of any Neural Network (NN) with cross-entropy loss over one-hot labels, which is the general case for classification ~\citep{lyu2020threats}. Several strategies have been discussed to defend these attacks including gradient perturbation, low precision, and gradient compression. Adding noise on gradients before sharing can prevent the leakage, but can also cause the model performance drop significantly. While half precision fails to protect, gradient compression successfully defends the attack with the pruned gradient is more than $20\%$. In addition, ~\citep{gradientscompression2017} discovered that $99.9\%$ of the gradient exchange in distributed stochastic gradient descent (SGD) are redundant, and then they proposed to use momentum correction, local gradient clipping, momentum factor masking, and warm-up training to preserve accuracy and overcome the staleness problem caused by reduced communication respectively. 

%Cryptology can also be used to prevent the information leakage ~\citep{homomorphicEncryption2018}. For example, ~\citep{bonawitz2017practical} proposed to use~\emph{Secure Aggregation} to compute an aggregate value (updates from clients) without revealing to others any information regarding the private value each client owns excepts what is learnable from the aggregated value itself. Several protocols have been developed in a series of refinements to achieve the goal of secure aggregation~\citep{bonawitz2017practical}. However, the security will be lost when some protocol is facing the honest-but-curious servers\footnote{Servers are assumed to extract the data of individuals; and yet they are honest in operations ~\citep{homomorphicEncryption2018}.} who are trying to learn as much as possible from messages they receive from clients. %For example, Protocol $0$ (Masking with One-Time Pads) can guarantee the perfect privacy for each client but it is sensitive to dropped users. Protocol $1$ (Dropped User Recovery using Secret Sharing) leverages $(t, n)$-threshold scheme\footnote{A $(t, n)$ secret-sharing scheme allows splitting a secret into $n$ shares, such that any subset of $t$ shares is sufficient to recover the secret, but given any subset of fewer than $t$ shares, the secret remains completely hidden.} to improve robustness. However, the security will be lost when Protocol $1$ is facing the honest-but-curious servers\footnote{Servers are assumed to extract the data of individuals; and yet they are honest in operations (~\cite{homomorphicEncryption2018}).} who are trying to learn as much as possible from messages they receive from clients. Protocol $2$ (Double-Masking to Thwart a Malicious Server) can guarantee the security even when the malicious server can reconstruct a client's perturbations. 

%~\citep{homomorphicEncryption2018} proposed to address the problem of information leakage to server in the Shokri-Shmatikov system ~\citep{Shokri2015} which only shares a part of local gradients with the server. By using additively homomorphic encryption, all gradients are encrypted and stored on the server. The additive homomorphic property enables the computation over the gradients and enjoys both security and accuracy. However, above approaches cannot be flexibly generalized to all algorithms and operations, and incur additional computation and design cost ~\citep{FDML2019}.

%Relatively earlier, differential privacy has also been applied to achieve a tradeoff between privacy and utility of the trained model ~\citep{DPDwork2006,NIPS2010DPPathak, Rajkumar2012DP}. Differential privacy was first proposed by ~\citep{DPDwork2006} to capture the increased risk to one’s privacy incurred by participating in a database. Differential privacy has now become a standard privacy model for statistics analysis with provable privacy guarantee ~\citep{dpZhao2018}. %Intuitively, given any dataset $D$ and $D'$, a mechanism satisfies differential privacy if its outputs are approximately the same for $D$ and $D'$, so that an adversary infers no more information from the outputs about the record owner in $D$ than $D'$ where the record is absent.

% There is also some work which does not require gradients exchange. For example, ~\cite{FDML2019} proposed a framework named as \emph{FDML} to achieve the goal of improving the predictive power of one party by leveraging additional features from other parties without requiring any party to share their local features or model parameters. %Each party is solely responsible for updating its own local model (can be arbitrary) parameters using its own mini-batch of local feature sets. For each record, it only needs to share the local prediction results to the central server (or other parties directly in a fully decentralized scenario). The server aggregates all the local prediction results from all parties and send the aggregated results to parties for updating their corresponding local parameters. An asynchronous SGD algorithm and a parameter server architecture are proposed to solve the optimization problem in \emph{FDML}, with theoretical convergence guarantees under bounded asynchrony. 
% One privacy concern of \emph{FDML} is that the labels have to be sent to all parties so each party can compute error gradients locally. For example, advertisers may want to treat these purchase and conversion labels as sensitive information and be reluctant to share these information with other parties. %To achieve a higher level of privacy, some additional differential privacy based methods can be applied to perturb local predictions before being uploaded to the server.

==> tex/algorithms/encrypted_bp.tex <==
\begin{algorithm}[H]
\SetAlgoLined
\KwIn{The passive party ($\mathcal{P}_p$) and active party ($\mathcal{P}_a$) own their own data $\mathcal{D}_p = (\mathcal{I}_p, \mathcal{X}_p)$ and $\mathcal{D}_a = (\mathcal{I}_a, \mathcal{Y}_a)$, respectively. Number of training epochs: {num\_{epoch}}. Learning rate $\eta$.}
\KwOut{$\mathcal{P}_a$ and $\mathcal{P}_p$ learn their model parameters $W_a$ and $W_b$, respectively}
\caption{Encrypted Back-propagation Algorithm}
\label{alg:encrypted_bp}
\tcp{\bf Initialization}
    $\mathcal{P}_a$ and  $\mathcal{P}_p$ initialize their corresponding model parameters $W_a$ and $W_b$, respectively. \\
    
    $\mathcal{P}_a$ initializes a secure homomorphic cryptosystem {\texttt {crypto}}.\\

\tcp{\bf Federated Model Training}
    \For{$k \le {num\_{epoch}}$}{
    $\mathcal{P}_p$ sends a batch of $\{(e_i^k, f^k(\mathcal{X}_i))\}$ to the $\mathcal{P}_a$, where $e_i^k$ is the sample id for data alignment. \\
    
    $\mathcal{P}_a$ generates the gradient $g^k$ depending on whether $e_i^k$ belongs to $\mathcal{P}_a$:
       $ g_i^k =
        \begin{cases}
        \frac{\partial \mathcal{L}}{\partial f^k(\mathcal{X}_i)} & \text{if $e_i^k \in \mathcal{I}_a$} \\
        \mathbf{0} & \text{otherwise}
        \end{cases}$ \\
        
    $\mathcal{P}_a$ uses {\texttt {crypto}} to encrypt $g^k$ and sends encrypted $[g^k]$ to $\mathcal{P}_p$. \tcp{ First Round Communication} \\ 
    
    $\mathcal{P}_p$ computes its local gradient $[g^k \nabla_{W_p} f^k(\mathcal{X})]$ in the cipher-space. \\
    
    $\mathcal{P}_p$ masks its local gradients by $[\frac{\partial {\mathcal{L}}}{\partial {W_p}}] = r^k \odot [g^k \nabla_{W_p}  f^k(\mathcal{X})]$ where $r^k$ is a randomly chosen non-zero value and $\odot$ denotes the Hadamard product. \\
    
    $\mathcal{P}_p$ sends the masked gradients $[\frac{\partial {\mathcal{L}}}{\partial {W_p}}]$ to $\mathcal{P}_a$ for decryption. \tcp{ Second Round Communication}  \\
    
    $\mathcal{P}_a$ uses {\texttt {crypto}} to decrypt $[\frac{\partial                              {\mathcal{L}}}{\partial {W_p}}]$ and     sends the decrypted $\frac{\partial             {\mathcal{L}}}{\partial {W_p}}$ to               $\mathcal{P}_a$. \tcp{Third Round Communication}  \\
  
   $\mathcal{P}_p$ uses the Hadmamard division to recover $\frac{\partial {\mathcal{L}}}{\partial {W_p}}$. \\
  
   $\mathcal{P}_a$ computes the gradients of its local parameters $\frac{\partial \mathcal{L}}{\partial W_a}$ in plaintext space. \\
    
   $\mathcal{P}_p$ and $\mathcal{P}_a$ update their local models with $\frac{\partial {\mathcal{L}}}{\partial {W_p}}$ and $\frac{\partial \mathcal{L}}{\partial W_a}$ respectively. 
  }
\end{algorithm}





==> tex/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{Despite that we include spectral and intersection membership leakage, we do not invent or promote it but merely use it as an evaluation metric. In addition, our proposed strategies can prevent leakage from these attacks.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{We provide code and instructions in the supplementary material. We include the preprocessing code for all the datasets (datasets are all public).}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Our experiments requires computing the performance for dozens of model training runs. It is computationally too demanding to compute error bars for every such training run by also doing multiple runs. In addition, we believe the results are consistent and convincing enough without additional error bars.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
     \answerYes{We provide such details in the Appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We use a model architecture proposed in a prior paper which we cite.}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tex/framework/convergence_proof.tex <==
\subsubsection{Convergence Proof}

==> tex/framework/fl_training_serving.tex <==

\subsection{Federated Model Training and Serving}
\label{sec:training_serving}

% After we leverage PSU to align the dataset and provide synthetic data using strategies as described in previous subsection, we can begin the federated model training. In this paper we focus on two parties learning a model for a binary classification problem over the domain $\calX \times \cbrck{0, 1}$. Here the passive and active parties want to learn a composition model $h \circ f$ jointly, where the raw features $X$ and $f: \calX \to \Real^d$ are stored on the passive party side while the labels $y$ and $h: \Real^d \to \Real$ is on the active party side. Let $\ell = h(f(X))$ be the logit of the positive class where the positive class's predicted probability is given by the sigmoid function. The loss of the model is given by the cross entropy. \kevin{Should this para be put in 2.1? Those settings are implictly assumed in early method subsection but no explanation. Better to put it at the beginning.} %Let $\ell = h(f(X))$ be the logit of the positive class where the positive class's predicted probability is given by the sigmoid function as follows: $\widetilde{p}_1 = 1/(1 + \exp(-\ell))$. The loss of the model is given by the cross entropy $L = \log(1 + \exp(-\ell)) + (1 - y)\ell$. 

To train the model using gradient descent, the passive party computes the cut layer embedding $f(X)$ with both synthetic and real raw features $X$ and sends it to the active party who will then complete the rest of computation (Forward).\footnote{
For the simplifying of the notation and derivation, we add no additional features in the active party to compute the logit. 
The data generation strategies can be adapted for other complicated settings.
}  Then the active party starts the gradient computation process by first computing the gradient of the loss with respect to the logit $\frac{dL}{d\ell} = (\widetilde{p}_1 - y)$. Here $y$ contains both synthetic and real labels. Using the chain rule, the active party can then compute the gradient of $L$ with respect to $h$'s parameters through $\ell$. In order to allow the passive party to learn $f$, the active party also computes the gradient of $L$ with respect to the input of the function $h$. We denote this gradient by $g$  (equality by chain rule). After receiving $g$ sent from the active party, the passive party can compute the gradient of $L$ w.r.t. $f$'s parameters (Backward). 

\begin{comment}
% \newcommand{\pp}{c}
  \begin{table*}[!ht]
  \centering
%   \begin{center}
    % \scriptsize
    \begin{tabular}{ cccccccccc }
      { Forward:} & $X$ & $\xrightarrow{\bm{f}}$ & $\bm{f}(X)$ & $\stackrel{\textrm{\scriptsize comm.}}{\Longrightarrow}$ & $\bm{f}(X)$ & $\xrightarrow{\bm{h}}$ &$\ell=h(f(X))$ & $\rightarrow$ & $\stackrel{\stackrel{\mbox{$y$}}{\downarrow}}{L}$ \\
      { Backward:} & & & $g$ & $\stackrel{\textrm{\scriptsize comm.}}{\Longleftarrow}$ & $g \coloneqq \nabla_{\bff(X)}L $ & $\leftarrow$ & $\frac{dL}{dl} = (\widetilde{p}_1 - y)$ & $\leftarrow$ & $1$ \\
      & & & $\downarrow$ & & & & $\downarrow$ & & \\
      & & & $f$'s param & & & & $h$'s param & & 
    \end{tabular}
%   \end{center}
    \caption{Communication diagram of model training ($\leftarrow$ and $\downarrow$ represent gradient computation using the chain rule).}
    \label{tab:model_training}
    \vspace{-0.15in}
  \end{table*}
\end{comment}
When $B$ examples are forwarded as a batch, the communicated features $f(X)$ and gradients $g$ will both be matrices of shape $\Real^{B \times d}$ with each row belonging to a specific example in the batch. It is important to note that here the gradients as rows of the matrix are gradients of the loss with respect to different examples' intermediate computation results but not the model parameters; therefore, no averaging over or shuffling of the rows of the matrix can be done prior to communication for the sake of correct gradient computation of $f$'s parameters on the passive party side.

% \xin{Why do we have the following paragraph? Is serving different from training?} \jk{i add the inference part here in case reader are curious. may add it to the appendix based on the space usage.}
For model inference,
suppose that the passive party would like to know the prediction of instance $i$ from the active party. The passive party only feeds $i$'s raw feature $x$ and computes $f(x)$. 
If no additional features are added in the active party to compute the logit,
then the active party directly computes $p_i = 1/(1 + exp(-h(f(x))))$ and sends $p_i$ to the passive party without knowing any ID information of $i$. 
Otherwise if additional features are needed for active party, the passive party can hide instance $i$ in a batch which both parties have agreements on. Then the serving process will be the as same as the forward process during the training phase. After receiving a batch of predictions from the active party, the passive party can select the corresponding prediction for $i$. \kevin{What does the above two paras try to present that is different from the normal VFL? Is it just logit shift? If so, can we merge it with 2.3.4? }




==> tex/trash.tex <==
\input{tex/algorithms/encrypted_bp}

Algorithm ~\ref{alg:encrypted_bp} is not secure as expected. $\mathcal{P}_p$ knows $\frac{\partial {\mathcal{L}}}{\partial {W_p}}$ and $\nabla_{W_p}  f^k(\mathcal{X})$ for each batch. A malicious passive party can estimate $g^k$ with least-squares solution by solving the linear matrix equation $g^k \nabla_{W_p}  f^k(\mathcal{X}) = \frac{\partial {\mathcal{L}}}{\partial {W_p}}$ ~\footnote{\url{ https://numpy.org/doc/stable/reference/generated/numpy.linalg.lstsq.html}}. The synthetic gradients can not be hided in the crowed if we set synthetic gradients be $\mathbf{0}$.


\subsubsection{Generate Synthetic Gradients from Real Gradients}

Suppose the passive party has two layers:

\begin{align*}
    Z_1 = W_1 X + b_1 \\
    A_1 = \sigma_1(Z_1) \\
    Z_2 = W_2 A_1 + b_2 \\
    A_2 = \sigma_2(Z_2) \\
\end{align*}

To be consistent with our previous notations, we have:

\begin{align*}
    \mathbf{f}(X) = A_2 \\
    \frac{\partial L}{\partial A_2} = g
\end{align*}

Then we have:

\begin{align*}
    \frac{\partial L}{\partial W_2} = g \frac{\partial A_2}{\partial Z_2}\frac{\partial Z_2}{\partial W_2} = g \frac{\partial A_2}{\partial Z_2}A_1 \\
    \frac{\partial L}{\partial b_2} = g \frac{\partial A_2}{\partial Z_2}\frac{\partial Z_2}{\partial b_2} = g \frac{\partial A_2}{\partial Z_2}
\end{align*}


\begin{align*}
    \frac{\partial L}{\partial W_1} = g \frac{\partial A_2}{\partial Z_2}\frac{\partial Z_2}{\partial A_1} \frac{\partial A_1}{\partial Z_1} \frac{\partial Z_1}{\partial W_1} = g \frac{\partial A_2}{\partial Z_2} \frac{\partial Z_2}{\partial A_1} \frac{\partial A_1}{\partial Z_1}X = g \frac{\partial A_2}{\partial Z_2} W_2 \frac{\partial A_1}{\partial Z_1}X \\
    \frac{\partial L}{\partial b_2} = g \frac{\partial A_2}{\partial Z_2}\frac{\partial Z_2}{\partial A_1} \frac{\partial A_1}{\partial Z_1} \frac{\partial Z_1}{\partial b_1} = g \frac{\partial A_2}{\partial Z_2} \frac{\partial Z_2}{\partial A_1} \frac{\partial A_1}{\partial Z_1}= g \frac{\partial A_2}{\partial Z_2} W_2 \frac{\partial A_1}{\partial Z_1}
\end{align*}

Both $\frac{\partial A_2}{\partial Z_2}$ and $\frac{\partial A_1}{\partial Z_1}$ are derivative of the activation functions $\sigma_2$ and $\sigma_1$ respectively. For example, if $\sigma_2$ is a sigmoid function, $\frac{\partial A_2}{\partial Z_2} = \sigma_2(Z_2)\sigma_2(1-Z_2)$. 

Suppose $K_1(X) = \frac{\partial A_2}{\partial Z_2} W_2 \frac{\partial A_1}{\partial Z_1}X$ and $K_2(X) = \frac{\partial A_2}{\partial Z_2}A_1$, we have:

$\frac{\partial L}{\partial W_1} = K_1(X^T) g$ and $\frac{\partial L}{\partial W_2} = K_2(X^T) g$

where $X \in \mathcal{R}^{n \times d_x}$, $K_1(X^T) \in \mathcal{R}^{k_1 \times n}$, $K_2(X^T) \in \mathcal{R}^{k_2 \times n}$, and $g \in \mathcal{R}^{n \times d_g}$.

\begin{align*}
    \frac{\partial L}{\partial W} = K(X^T)g    
\end{align*}

For each element $\frac{\partial L}{\partial W}[i][j]$ ($\forall i, j, 0 \le i < k, 0 \le j < d_g$) in $\frac{\partial L}{\partial W}$:

\begin{align*}
    \frac{\partial L}{\partial W}[i][j] = K(X^T)[i][0] \times g[0][j] + K(X^T)[i][1] \times g[1][j] + ... + K(X^T)[i][n-1] \times g[n-1][j] \\ 
  = \sum_{t=0}^{n-1} K(X^T)[i][t] \times g[t][j]  
\end{align*}

For each row $i$ in $g$, if its corresponding instance ID $id_i \in I_a$, the corresponding label $y_i$ is observed and its corresponding gradients $g[i]$ are real. Otherwise, the corresponding label $y_i$ is not observed and its corresponding gradients $g[i]$ are synthetic. 

Hence:

\begin{align*}
    \frac{\partial L}{\partial W}[i][j] = \sum_{t, {id}_t \in I_a} K(X^T)[i][t] \times g[k][j] +  \sum_{t', {id}_{t'} \notin I_a} K(X^T)[i][t'] \times g[t'][j] \\
    = \nabla W_{obs}[i][j] + \nabla W_{syn}[i][j]
\end{align*}


where $\nabla W_{obs}$ is the real gradients generated from the observed instances, and $\nabla W_{obs}$ is the synthetic gradients for instances which are not in the active party. The synthetic gradients should have little effect on the model parameters updates. $\nabla W_{syn}$ should be close to $0$ or $\nabla W_{obs}$. 

The most straightforward way to generate synthetic gradients is by setting $g_{syn} = \mathbf{0}$ so that $\nabla W_{syn} = \mathbf{0}$ and the existence of the synthetic gradients does not affect the relevant computed result. However, the passive party can breach the ID privacy by checking with row in $g$ is $\mathbf{0}$. 


\input{tex/framework/convergence_proof}


\subsubsection{Encrypted Back-propogation is NOT Secure as Expected}

Liu et al. ~\cite{lzw20} proposed an encryption-based approach to train an asymmetrical vertical federated logistic regression model to protect the sample IDs privacy of the weak party. Inspired by their work, we propose to encrypt the back-propogation process of neural networks to prevent the passive party seeing the communicated gradients directly. Due to the linearity of the back-propogation, homomorphic encryption such as Paillier can be applied to our scenario. 





\subsubsection{\textbf{Understanding Synthetic Features with Smooth Label}}

We can understand the synthetic feature strategy by considering that our real input has a label distribution, not a one-hot label. Suppose the $x$'s real label is $y$ and feature missing ratio is $\alpha$. With our synthetic features generation strategy, the label distribution is represented as: $q(y') = \alpha p(y=y') + (1-\alpha) 1[y=y']$ where $y'=0$ or $1 $ and $p(y)$ is the label marginal distribution.

To correctly use this information, one way is to use the soft cross entropy loss function: $E_q [\log p(y|x)] = -[q(y'= 1)\log p(y=1|x) + q(y'=0)\log p(y=0|x)]$. However, this is difficult to use in our vertical FL settings. 
We may approximate the soft cross entropy loss function by sampling from it: $E_q [\log p(y|x)] \approx \frac{1}{S}\sum_{s=1}^S \log p(y_s|x) $ where  $ y_s\sim q(y')$.

This is equivalent with the approach we are using to generate synthetic features. To have this approximation work as desired,  $S$ can't be too small.  $S$ can be viewed as the number of duplicated times of a real feature, which is equal to $k * \frac{\alpha}{1-\alpha}$ on average where  $k$ is the number of running epochs. Hence increasing  $k$ is beneficial for getting a good approximation.

To have a better understanding, we use an example to show how to compute the smooth label for each instance. Here $ \alpha$ represents feature missing ratio (e.g. $95\%$) and $\beta$ is positive label ratio ($10\%$). Given a real positive instance $(x, y)$ with $y=1$, with synthetic feature generation strategy, feature $x$ is duplicated by $\frac{\alpha}{1-\alpha} $ times on average in an epoch. Among all the duplicates, we have:
\begin{itemize}
    \item Number of positive random labels for  $ x $ :  $  \frac{\alpha \beta}{1-\alpha} $ 
    \item Number of negative random labels for  $ x $ :  $  \frac{\alpha (1-\beta)}{1-\alpha} $
\end{itemize}
 
Remember we still have one positive label for the original  $(x, y)$. Hence, overall, the number of positive random labels for $x$ is $  \frac{\alpha \beta}{1-\alpha}+1$.
Then the soft label for $(x, y)$ is:  $y=[\frac{ \frac{\alpha (1-\beta)}{1-\alpha}}{ \frac{\alpha }{1-\alpha}+1}, \frac{ \frac{\alpha \beta}{1-\alpha}+1}{ \frac{\alpha }{1-\alpha}+1} ] = [\alpha(1-\beta), 1-\alpha+ \alpha\beta)]$. It's worth mentioning that $ 1-\alpha+\alpha\beta > \beta $  <=>  $ (1-\alpha)(1-\beta)>0$, which means the positive value is still larger than the original marginal probability of being positive  $\beta$.

Similarly, we can compute the soft label for a real negative instance with  $y=0$ as $y=[\frac{ \frac{\alpha (1-\beta)}{1-\alpha}+1}{ \frac{\alpha }{1-\alpha}+1}, \frac{ \frac{\alpha \beta}{1-\alpha}}{ \frac{\alpha }{1-\alpha}+1} ] = [1-\alpha\beta, \alpha\beta)]$ where $1-\alpha\beta > 1-\beta$ which means the negative value is still larger than the original marginal probability of being negative $1-\beta$.

Suppose the missing ratio $\alpha = 0.95$ and positive ratio $\beta=0.25$ , then we have smooth label for positive instances as  $[0.95*0.75, 1-0.95+0.95*0.25] = [0.7125, 0.2875]$ and negative ones as $[1-0.95*0.25, 0.95*0.25] = [0.7625, 0.2375]$ respectively.

\subsubsection{Logits Shift for Synthetic Labels and Features}
$$\begin{aligned}
p(y=1|x',\theta) = (1-\alpha) \cdot (1-\beta) \cdot g(y=1|x) + (1-\beta) \cdot  \alpha \cdot p(y=1|\theta) 
\end{aligned}$$

$$\begin{aligned}
\frac{1}{1+e^{-h(x, \theta)}} = (1-\alpha) \cdot (1-\beta) \cdot \frac{1}{1+e^{-g(x, \theta)}} + (1-\beta) \cdot \alpha \cdot p
\end{aligned}$$

Thus:

\begin{align}
h(x,\theta) = -log(\frac{1}{\frac{(1-\alpha)\cdot (1-\beta)}{1+e^{-g(x,\theta)}} + (1-\beta)\cdot \alpha \cdot p} - 1)    
\end{align}



\subsubsection{Privacy Analysis of Synthetic Labels}

Under the setting of vertical FL, the passive party has access to:

\begin{itemize}
    \item The raw features $X$
    \item The cut layer embedding $f(X)$
    \item The gradients of the cut layer embedding received from the active party $g$. $g$ is computed by the active party with synthetic generation strategy \synzero{} and its variants. 
\end{itemize}

We analyze how can the passive party leverage the above information to check the existence of sample IDs in the active party.

As described in Section ~\ref{sec:synthetic_features}, the passive party samples features from historical data to generate synthetic features. One privacy concern we have here is that it's possible different sample IDs share the same synthetic feature $x_i$ (a real feature of $id_i \in \mathcal{I}_p$) and hence the passive party sends the same feature to the active party multi-times. An curious passive party may record the corresponding feature's gradients and compare. If the active party owns $id_i$ and by chances $y_i = 1$. Then the passive party can see the difference between gradients and then infer the active party owns $id_i$ with $y_i = 1$. However, we don't think it's a privacy concern here, since: 
\begin{itemize}
    \item It's highly impossible that all the duplicate features $x_i$ and $x_i$ itself occur in the same mini-batch. Let alone the active party happens to own $id_i$ with $y_i = 1$.
    \item With time increasing, the network is evolving. It's natural to see one raw feature has different cut layer embeddings at different times.
\end{itemize}


\subsubsection{Potential Privacy Concerns of Synthetic Features}
The active party has access to:
    \begin{itemize}
        \item The cut layer embedding $f(X)$
        \item Label information $Y$
        \item The gradients $g$ of the cut layer embedding sending to the passive party.
    \end{itemize}
    
In this section, we analyze some potential privacy concerns on distinguishing synthetic cut layer embed from real ones by leveraging above information.
   
   
Take an extreme case for example, the active party may see $k$ different sample IDs share the same cut layer embedding in one mini-batch. Then the active party knows that only one of them is real and the rest of them are synthetic. The probability of guessing right is $1/k$. It's worth mentioning that the random guess probability is $1-\alpha$. Based on the law of large numbers, both numbers are equivalent. Hence our synthetic strategy leaks no additional information.
